Inverse Problems and Data Assimilation

We provide a clear and concise introduction to the subjects of inverse problems and data assimilation, and their inter-relations. The first part of our notes covers inverse problems; this refers to the study of how to estimate unknown model parameters from data. The second part of our notes covers data assimilation; this refers to a particular class of inverse problems in which the unknown parameter is the initial condition (and/or state) of a dynamical system, and the data comprises partial and noisy observations of the state. The third and final part of our notes describes the use of data assimilation methods to solve generic inverse problems by introducing an artificial algorithmic time. Our notes cover, among other topics, maximum a posteriori estimation, (stochastic) gradient descent, variational Bayes, Monte Carlo, importance sampling and Markov chain Monte Carlo for inverse problems; and 3DVAR, 4DVAR, extended and ensemble Kalman filters, and particle filters for data assimilation. Each of parts one and two starts with a chapter on the Bayesian formulation, in which the problem solution is given by a posterior distribution on the unknown parameter. Then the following chapter specializes the Bayesian formulation to a linear-Gaussian setting where explicit characterization of the posterior is possible and insightful. The next two chapters explore methods to extract information from the posterior in nonlinear and non-Gaussian settings using optimization and Gaussian approximations. The final two chapters describe sampling methods that can reproduce the full posterior in the large sample limit. Each chapter closes with a bibliography containing citations to alternative pedagogical literature and to relevant research literature. We also include a set of exercises at the end of parts one and two. Our notes are thus useful for both classroom teaching and self-guided study.

==> lectures/Assignment3.tex <==
\chapter*{\Huge{\sffamily{STAT 31550 -- Assignment 3}}}
\label{ch:DAExercises}
\addcontentsline{toc}{chapter}{Exercises}

\noindent {\bf Exercise 1} ({\sffamily{Filtering and Smoothing: Scalar Linear-Gaussian Setting}}) 
Consider the scalar stochastic dynamics and observation models given by 
\begin{align*}
v_{j+1}&=a v_j+ \xi_j, \quad \quad \xi_j\sim \Nc(0,\sigma^2),  \quad \quad v_0 \sim \Nc(m_0,c_0^2), \\
y_{j+1} &= v_{j+1} + \eta_{j+1}, \quad \quad \eta_{j+1} \sim \Nc(0,\gamma^2),
\end{align*}
with $v_0$ independent of the \index{i.i.d.}i.i.d.
sequences \(\{\xi_j\}\) and  \(\{\eta_j\}\).

\begin{enumerate}
    \item Set $a = 1.25,$ $\sigma^2 = 0.5,$ $m_0 = 1,$ $c_0^2 = 1$ and $\gamma^2 =0.1.$ Generate synthetic data $\{y_j\}_{j=1}^J$ with $J = 10$ from this model following these steps: 
    \begin{enumerate} 
    \item  Sample $v_0^\dagger \sim \Nc(1, 1).$ 
    \item For $j=0, \ldots, 9,$ sample $v_{j+1}^\dagger \sim \Nc(1.25 v_j^\dagger, 0.5)$. 
    \item For $j=0, \ldots, 9$, sample $y_{j+1} \sim \Nc(v_{j+1}^\dagger, 0.1).$ 
    \end{enumerate}
    We interpret $\{v_j^\dagger\}_{j=0}^{10}$ as the true signal underlying the synthetic data $\{y_j\}_{j=1}^{10}$. 
    \item For the synthetic data generated above, find the filtering distributions $\pi_j(v_j) = \mathbb{P}(v_j|y_1, \ldots, y_j)$ for $j=0, 1, \ldots, 10$ using the Kalman filter. Find the smoothing distribution $\mathbb{P} (\{v_j\}_{j=0}^{10} | \{y_j\}_{j=1}^{10})$ using the Kalman smoother. 
    \item Plot, for discrete time $1\le j \le 10,$  the mean of the filtering and smoothing distributions, together with the true signal and the observations.
\end{enumerate}


\noindent {\bf Exercise 2} ({\sffamily{The Pendulum Problem}}) 
The dynamics of a pendulum are characterized by the following linear system:
$$\ddot{u} + \delta{\dot{u}} + \sin(u) = 0,$$
where $u(t)$ denotes the location of the pendulum, $\dot{u}(t)$ denotes the velocity and $\delta$ is a scalar parameter.
\begin{enumerate}
\item Show that the dynamical system can be equivalently written as:
$$\frac{\mathrm{d}}{\mathrm{d}t} \Big[\frac{1}{2}\dot{u}^2 - \cos(u)\Big] = -\delta\dot{u}^2.$$
Justify that for $\delta \geq 0$ the solution will not blow up in finite time. What happens when $\delta = 0$?
\item  Show that the dynamical system can be equivalently expressed by the system of equations:
\begin{eqnarray}
\begin{cases}
\dot{u} = w,\\
\dot{w} = -\delta{w} - \sin(u) ,
\end{cases}
\label{eqn:diff}
\end{eqnarray}
with $v =( u , w)^\top$.  Let $\Psi(v)$ denote the solution of \eqref{eqn:diff} at time $t = 0.2$ with initial condition $v.$ Set  $v_0 = (u^0,w^0)^\top = (\pi/4,0)^\top$ and consider the deterministic dynamics model and observation model given by
\begin{align}
\begin{split}\label{eqn:diff2}
v_{j+1} &= \Psi(v_{j}), \\
y_{j+1} &= u_{j+1} + \eta_{j+1}, \quad \eta_j \sim \mathcal{N}(0, \gamma^2) \index{i.i.d.} \text{ i.i.d.}
\end{split}
\end{align}
Set $\gamma^2 = 0.01$ and $\delta = 0.1$. Solve numerically the differential equation \eqref{eqn:diff2} and obtain $20$ observations $\{y_j\}_{j=1}^{20}$. Plot these values. 
\item Letting $H = \begin{pmatrix} 1 & 0 \end{pmatrix}$, recall that 3DVAR obtains estimates $m_{j+1}$ of the signal from the following sequential computations: 
\begin{eqnarray*}
m_{j+1} = (I - KH)\Psi(m_j) + Ky_{j+1},
\end{eqnarray*}
a tradeoff between fitting to data and getting accurate dynamics. Here the matrix $K$ satisfies the relations:
\begin{eqnarray*}
S = H \widehat{C} H^\top + \gamma^2, ~~~ K = \widehat{C} H^\top S^{-1},
\end{eqnarray*}
with $\widehat{C} \in \mathbb{R}^{2\times{2}}$  to be specified. Consider initializing 3DVAR from $m_0 = (0,0)^\top$ and suppose that $\widehat{C}$ is chosen to be a diagonal matrix. In this problem, show that there is only one degree of freedom. Play around with this parameter to find one that gives you a small $\sum_{j = 1}^{20} |v_{j} - m_{j}|$. (This is a bit of an open ended problem. We want you to play around a bit!). 
\item Repeat items 2 and 3 above with the observations being on the state $w$ instead of $u$, e.g. $y_{j+1} = w_{j+1} + \eta_{j+1}$. What do you notice?
\item Starting with $N \in\{5,20,50,100\}$ random particles, sampled from a Gaussian $\Nc(0, I_2),$  apply particle filtering and report the effective sample size after each iteration of the dynamics. What do you observe?
\item What is the advantage of particle filtering for this problem over 3DVAR? What about a disadvantage?\end{enumerate}

\bigskip

\noindent {\bf Exercise 3} ({\sffamily{Estimation of Model Parameters: the EM Algorithm}}) 
Consider \index{stochastic dynamics model}stochastic dynamics and \index{data model}data models given by 
\begin{align}
        v_{j+1} &= \Psi_\theta(v_j) + \xi_j, && \xi_j \sim \Nc(0, \Sigma) \index{i.i.d.} \text{ i.i.d.}, \label{eq:SSM1}\\
        y_{j+1} &= Hv_{j+1} + \eta_{j+1}, && \eta_j \sim \Nc(0, \Gamma) \index{i.i.d.}\text{ i.i.d.}, \label{eq:SSM2}
\end{align}
with \(v_0 \sim \Nc(m_0, C_0)\) independent of the independent \index{i.i.d.}i.i.d.
sequences \(\{\xi_j\}\) and  \(\{\eta_j\}\). Here the vector $\theta \in \R^p$ parameterizes the dynamics. 
For a given and fixed integer $J,$ set
$\V := \{v_0, \ldots, v_J\}$ and  $\Y := \{y_1, \ldots, y_J\}.$
We seek to find $\theta$ that maximizes the \index{likelihood}likelihood function of $\theta$ given the observed data $Y$:
\begin{equation}
\Prob(Y | \theta) = \int \Prob (V, Y |\theta) \, dV.
\end{equation}
Here and below $\Prob (Y | \theta)$ denotes the pdf of $Y$ given that the dynamics map $\Psi_\theta$ in \eqref{eq:SSM1} are parameterized by $\theta;$ $\Prob(V,Y |\theta)$ is defined similarly. 
 
 \begin{enumerate}
\item Show that the joint distribution of $V$ and $Y$ admits the characterization
\begin{align}\label{eq:joint}
\begin{split}
\hspace{-0.5cm} \log & \Prob(V,Y | \theta) 
 =  -  \frac{1}{2} \displaystyle{\sum_{j=0}^{J-1}}|y_{j+1} - Hv_{j+1}|_{\Gamma}^2 
 -  \frac{1}{2}|v_0-m_0|^2_{C_0} - \frac{1}{2}  \sum_{j=0}^{J-1} |v_{j+1} - \Psi_\theta(v_j)|^2_{\Sigma}  + c,
\end{split}
\end{align}
where $c$ is a constant independent of $V,$ $Y$ and $\theta.$


\item Show that, for any pdf $q$ with compatible support, it holds that 
\begin{equation*}
\log \Prob (Y | \theta) = \mathcal{L}(q, \theta) + \dkl \bigl( q \| \Prob(V|Y,\theta)\bigr),
\end{equation*}
where 
$$\mathcal{L}(q, \theta) := \int\log\biggl( \frac{\Prob (V, Y| \theta)}{q(V)} \biggr) \, q(V)  \, dV.$$

\item 
You will now derive an iterative algorithm to maximize the likelihood.
Given the current iterate $\theta_\ell,$ we define  $\theta_{\ell+1}$ in two steps, maximizing in turn the two components of the lower bound $\mathcal{L}(q, \theta)$:
\begin{enumerate}
\item First, show that $q_\ell(V) = \Prob(V|Y,\theta_\ell)$ maximizes the lower bound $\mathcal{L}(q, \theta_\ell)$  over pdf $q.$  
\item Second, you will obtain $\theta_{\ell + 1}$ by maximizing the lower bound  $\mathcal{L}(q_\ell, \theta)$ over $\theta.$ Show that the quantity to maximize is the expected value of the joint log-density $\log  \Prob (V, Y | \theta)$ with respect to $q_\ell(V) = \Prob(V|Y, \theta_\ell).$
\end{enumerate}

Combining these two steps you have derived the Expectation Maximization \index{EM}(EM) algorithm, summarized below. 

\begin{algorithm}
\caption*{\label{alg:EM}{\bf Algorithm}  Expectation Maximization}
\begin{algorithmic}[1]
%\vspace{0.1in}
\STATE {\bf Input}:  Initialization $\theta_0.$
\STATE For $\ell = 0, 1, \ldots, L-1$ do the following expectation and maximization steps:
\STATE {\bf E-Step}: Compute 
\begin{align*}
\Expect^{V \sim  \Prob(V|Y, \theta_\ell)} \Bigl[ \log \Prob(V, Y | \theta) \Bigr]= \int \log \Prob(V, Y | \theta) \Prob(V|Y, \theta_\ell) \, dV. 
\end{align*}
\vspace{-0.5cm}
\STATE{{{\bf M-Step}}}: Compute 
\begin{equation*}
\theta_{\ell+1} = \arg \max_\theta \Expect^{V \sim  \Prob(V|Y, \theta_\ell)} \Bigl[ \log \Prob(V, Y | \theta) \Bigr].
\end{equation*}
%and replace $\ell$ by $\ell+ 1.$
\STATE{\bf Output}: Parameter $\theta^L.$
\end{algorithmic}
\end{algorithm}
\FloatBarrier

\item
Let $\{\theta_\ell \}_{\ell = 0}^{L-1}$ be the iterates of the EM algorithm. Show that, for $0 \leq \ell \leq L-1,$ it holds that 
\begin{equation}\label{eq:decreaselikelihood}
\log \Prob(Y | \theta_\ell) \le \log \Prob (Y | \theta_{\ell + 1}).
\end{equation}


\begin{remark}
\label{rem:em}
As a consequence of \eqref{eq:decreaselikelihood} it is possible to deduce ---under mild assumptions--- that the iterates $\theta_\ell$ of the \index{EM}EM algorithm converge, as $\ell \to \infty,$ to a local maximizer of the \index{likelihood}likelihood function. It is important to note, however, that the expectation in the E-step and the \index{optimization}optimization in the M-step are often intractable. \index{Monte Carlo}Monte Carlo, \index{filtering}filtering, or \index{smoothing}smoothing algorithms may be employed to approximate the E-step, and \index{optimization}optimization algorithms to approximate the M-step. Such approximations can cause loss of monotonicity and convergence guarantees. 
\end{remark}
\end{enumerate}

\bigskip

\noindent {\bf Exercise 4} ({\sffamily{EM Algorithm with Ensemble Kalman Filter}}) 
Consider the scalar stochastic dynamics and observation models given by 
\begin{align*}
v_{j+1}&= \theta v_j+ \xi_j, \quad \quad \xi_j\sim \Nc(0,\sigma^2),  \quad \quad v_0 \sim \Nc(m_0,c_0^2), \\
y_{j+1} &= v_{j+1} + \eta_{j+1}, \quad \quad \eta_{j+1} \sim \Nc(0,\gamma^2),
\end{align*}
with $v_0$ independent of the \index{i.i.d.}i.i.d. sequences \(\{\xi_j\}\) and  \(\{\eta_j\}\). Generate synthetic data $\{y_j\}_{j=1}^{10}$ from this model as in Exercise 1 using parameter $\theta^\star = 1.25.$ You will derive an EM algorithm to find $\theta^\star.$ Notice that the methodology you will derive is applicable in nonlinear settings. 
\begin{enumerate}
    \item Implement an ensemble Kalman filtering algorithm with $N = 100$ particles, so that given parameter $\theta_\ell$ it outputs an ensemble $\{v_j^{(n)}\}_{n=1}^{100}$ for discrete time $j = 0, 1, \ldots, 10.$  
    \item Using this ensemble Kalman filtering algorithm with parameter $\theta_\ell$, derive an (approximate) EM algorithm by setting 
    $$\theta_{\ell +1} = \arg \max_\theta \frac{1}{N} \sum_{n=1}^N \log \Prob(V^{(n)}, Y | \theta), $$
    where we define
      \begin{align*}
\begin{split}
\hspace{-0.5cm} \log  \Prob(V^{(n)},Y | \theta)  
 =  -  \frac{1}{2 \gamma^2} \displaystyle{\sum_{j=0}^{9}}|y_{j+1} - v_{j+1}^{(n)}|^2
 -  \frac{1}{2 c_0^2}|v_0^{(n)} - m_0|^2 - \frac{1}{2 \sigma^2}  \sum_{j=0}^{9} |v_{j+1} - \theta v_j^{(n)}|^2.
\end{split}
\end{align*}
    Implement this EM algorithm with an initialization $\theta_0 = 1.5$ to recover $\theta^\star.$
\end{enumerate}


\bigskip

\noindent {\bf Exercise 5} ({\sffamily{Likelihood: Linear-Gaussian Setting}}) 
 Suppose that, for each $0 \le j \le J-1,$ the predictive distribution $\Prob (v_{j+1}| Y_j, \theta)$ of the stochastic dynamics and data models \eqref{eq:SSM1} and \eqref{eq:SSM2} is \index{Gaussian}Gaussian with mean $\widehat{m}_{j+1}(\theta)$ and covariance $\widehat{C}_{j+1}(\theta).$ Show that then the \index{likelihood}log-likelihood function admits the following characterization 
\begin{equation*}
\log \Prob (Y | \theta) = - \frac12 \sum_{j = 0 }^{J-1} |y_{j+1} - H\widehat{m}_{j+1}(\theta)|_{S_{j+1}(\theta)}^2 - \frac12 \sum_{j=0}^{J-1} \log \text{{det}} \bigl(S_{j+1}(\theta)\bigr),
\end{equation*}
where $S_{j+1}(\theta) = H \widehat{C}_{j+1}(\theta) H^\top + \Gamma.$

\bigskip



    










==> lectures/Lecture14.tex <==
\chapter{\Large{\sffamily{Blending Inverse Problems and Machine Learning}}}
\label{ch:IPML}


In this chapter we study the use of \index{machine learning}machine 
learning\index{machine learning} in inverse problems. 
We have already seen ideas from \index{machine learning}machine learning, such
as \index{gradient descent!stochastic}stochastic gradient descent (Chapter \ref{chap:optimization})
and the \index{variational!formulation of Bayes theorem}variational formulation of \index{Bayes theorem}Bayes theorem (Chapter \ref{ch4}).
However, in this chapter we will embed \index{machine learning}machine learning into the formulation of the \index{inverse problem}inverse problem itself. 

The chapter is organized as follows: the first two sections discuss
key ideas from machine learning; the next three show their
application to \index{inverse problem}inverse problems.  
Section \ref{sec:FA} discusses the \index{supervised learning}supervised learning 
task of approximating a map from input-output pairs. Three families of methods 
for function approximation are considered: \index{neural network}neural networks, \index{random features}random features, 
and \index{Gaussian!process}Gaussian processes. In Section \ref{sec:MT} 
we focus on \index{unsupervised learning}unsupervised learning. Given samples 
from a target pdf, we introduce a range of generative models that enable 
the generation of new approximate samples from the target pdf by transforming 
samples from an easy-to-sample reference pdf. In Section \ref{sec:LForward} 
we show how approximate \index{forward!map}forward maps, found using
supervised learning,  may be used to 
speed-up \index{MCMC}MCMC while retaining accurate \index{posterior}posterior approximation.  
Section \ref{sec:LP} investigates the use of unsupervised techniques to recast 
a \index{Bayesian!inverse problem}Bayesian inverse problem with a given 
\index{prior}prior into an equivalent \index{inverse problem}inverse problem with an easy-to-sample prior; in particular, this may be used when prior information is
available only in the form of samples. 
Finally, Section \ref{sec:LPrtoPo} considers (unsupervised)
transport methods to learn the map from \index{prior}prior 
to \index{posterior}posterior. 
The chapter closes in Section \ref{sec:IPMLBib} with extensions and bibliographical remarks. 


\
\section{\index{supervised learning} Supervised Learning}
\label{sec:FA}
This section is concerned with the \index{supervised learning}{\em supervised learning} task of determining a function $\psid: D \subseteq \R^d \to \R$ from data in the form of input-output
pairs from the map. The codomain of $\psid$ may have finite cardinality (classification) or infinite cardinality (regression). We focus on regression since, as we will see in Subsection \ref{sec:LForward}, this task arises naturally in the context of learning forward maps for inverse problems. We assume that we have available to us data in the form 
\begin{align}
\label{eq:data}
\Bigl\{\un,\psid(\un) + \sqrt{\lambda} \xi_i^{(n)} \Bigr\}_{n=1}^N,
\end{align}
where $\xi^{(n)}$ is an \index{i.i.d.}i.i.d. mean zero noise process. The parameter $\lambda \ge 0$ allows us to consider noiseless data ($\lambda = 0)$ and noisy data $(\lambda >0).$
Since the goal is to determine $\psid$ we are concerned with function 
 \index{approximation}approximation, and to that end we will study three approaches to parameterize and learn functions: \index{neural network}neural networks (Subsection \ref{ssec:NN}), \index{random features}random features (Subsection  \ref{ssec:RF}), and Gaussian processes (Subsection \ref{ssec:GP}). 
We will concentrate on the noiseless case $\lambda = 0$, but will briefly mention the noisy case $\lambda >0$ in the context of \index{random features}random features and \index{Gaussian!process}Gaussian processes. 

Throughout, we assume that the data $\{\un\}_{n=1}^N$ 
are generated \index{i.i.d.}i.i.d. from pdf $\Upsilon(u)$, supported on $D \subseteq \R^d.$ We let $\hm$ denote the Hilbert space 
of real-valued functions on $D$ 
with inner-product and induced norm
$$\la \psi, \phi \ra_{\hm}=\int_{D} \psi(u)\phi(u)\Upsilon(u) \,du, \quad \|\psi\|_{\hm}^2=\la \psi,\psi \ra_{\hm}.$$
Thus
\begin{equation}\label{eq:norm}
\|\psi\|_{\hm}=\Bigl( \int_D \psi(u)^2  \Upsilon(u) \, du\Bigr)^{\frac12}.
\end{equation}
If $\Upsilon$ is the uniform distribution on bounded domain
$D \subseteq \R^d,$  we write the Hilbert space as $H = L^2(D);$ the norm and
inner-product are then denoted with $H$ as suffix.

In practice, the pdf $\Upsilon$ is typically unknown but may be approximated by the empirical density $\mn$ of the data $\{\un\}_{n=1}^N$, given by
\begin{align*}
\mn(u)=\frac{1}{N} \sum_{n=1}^N \delta(u-\un).
\end{align*} 
We may then define an empirical approximation of $\|\psi\|_{\hm}$
by replacing $\Upsilon$ by $\mn$ in \eqref{eq:norm} to obtain
$$\|\psi\|_{\hmn}=\Bigl( \frac{1}{N} \sum_{n=1}^N \psi(\un)^2 \Bigr)^{\frac12}.$$


The task of finding $\psid$ from data may be cast as a linear
\index{inverse problem}inverse problem, but this is not the 
connection to \index{inverse problem}inverse problems
that we will emphasize in this chapter; rather we will concentrate on
the use of \index{supervised learning}supervised learning, and variants, to formulate fast
approximate \index{Bayesian!inversion}Bayesian inverse methods, based on learning the 
log-likelihood\index{likelihood} or learning 
the forward model\index{forward!model}. 






%\begin{comment}
%%\as Introduce $L^2$ briefly. Say that regression requires pointwise evaluation.
%%\nc
%We focus on the \index{supervised learning}{\em supervised learning} task of determining 
%function a $\psid: \R^d \to \R$ from data in the form of input-output
%pairs from the map. Specifically, we assume that we have
%available to us data in the form 
%\begin{align}
%\label{eq:data}
%\bigl\{\un,\psid(\un) \bigr\}_{n=1}^N.
%\end{align}
%Natural generalizations include cases where
%$\psid: X \to Y$ with $X,Y$ being general Euclidean spaces
%(regression) and where $X$ is a Euclidean space and $Y$ a
%set of finite cardinality (classification). Furthermore, the
%case where the output data only satisfies $\yn \approx \psid(\un)$
%is also of interest. For example we may assume that
%\begin{equation}
%\label{eq:review}
%\psid(\un)=\psi\bigl(u^{(n)}\bigr)+\sqrt{\lambda}\xi^{(n)},
%\end{equation}
%where $\xi^{(n)}$ is an \index{i.i.d.}i.i.d. mean zero noise process.
%For expository purpose we assume 
%that $X=\R^d$ and $Y=\R$. We concentrate on the case
%$Y=\R$ and $\yn=\psid(\un)$ in our discussion of \index{neural network}neural networks. 
%In the context of
%\index{random features}random features and \index{Gaussian!process}Gaussian processes we discuss the noisy case. 
%Since the goal is to determine $\psid$ we are really concerned with function 
%approximation on Euclidean spaces. \index{approximation}
%We assume that data $\{\un\}_{n=1}^N$ 
%is generated \index{i.i.d.}i.i.d. from pdf $\Upsilon(u)$, supported on $D \subseteq \R^d.$ We let $\hm$ denote the Hilbert space 
%of real-valued functions on $D$ 
%with inner-product and induced norm
%$$\la \psi, \phi \ra_{\hm}=\int_{D} \psi(u)\phi(u)\Upsilon(u) \,du, \quad \|\psi\|_{\hm}^2=\la \psi,\psi \ra_{\hm}.$$
%Thus
%$$\|\psi\|_{\hm}=\Bigl( \int_D \psi(u)^2  \Upsilon(u) \, du\Bigr)^{\frac12}.$$
%It is of interest to define the empirical density $\mn$, given by
%\begin{align*}
%\mn(u)=\frac{1}{N} \sum_{n=1}^N \delta(u-\un).
%\end{align*} 
%We may then define empirical approximation of $\|\psi\|_{\hm}$, simply 
%replacing $\Upsilon$ by $\mn$ to obtain
%$$\|\psi\|_{\hmn}=\Bigl( \frac{1}{N} \sum_{n=1}^N \psi(\un)^2 \Bigr)^{\frac12}.$$
%In the case where $\Upsilon$ is \ds the uniform distribution on a bounded domain
%$D \subseteq \R^d$ \nc  we write the Hilbert space as $H = L^2(D)$ and norm and
%inner-product are denoted with $H$ as suffix.
%
%%\as I worry that $\Upsilon$ looks too much like $v$ in this font? \nc
%
%The task of finding $\psid$ from data may be cast as a linear
%\index{inverse problem}inverse problem, but this is not the 
%connection to \index{inverse problem}inverse problems
%that we will emphasize in this chapter; rather we will concentrate on
%the use of \index{supervised learning}supervised learning, and variants, to formulate fast
%approximate \index{Bayesian!inversion}Bayesian inverse methods, based on learning the 
%log-likelihood\index{likelihood} or learning 
%the forward model\index{forward!model}. 
%\end{comment}


\subsection{\index{neural network} Neural Networks}\label{ssec:NN}
A \index{neural network}neural network is a parametric family of functions. By use of the data a value of the parameter may be chosen so as to determine an approximation of $\psid.$
To define a \index{neural network}neural network we introduce
$\Theta \subseteq \R^{d_\theta}$ and then $\psi: \R^d \times \Theta \to \R$
via the iteration
\begin{align}
\label{eq:dnn}
\psi_0(u;\theta)&=u,\\
\psi_{\ell+1}(u;\theta)&=\sigma\bigl(W_{\ell}\psi_{\ell}(u; \theta)+b_\ell\bigr), \quad
\ell=0,\dots, L-1,\\
\psi(u;\theta)&=\beta^\top \psi_{L}(u; \theta).
\end{align}
In this definition, for $\ell \in \{0,\ldots, L-1\}$,
$W_{\ell}:\R^{d_{\ell+1}\times d_{\ell}}, b_{\ell} \in \R^{d_{\ell+1}}$
and $\beta \in \R^{d_{L}};$ together these matrices and vectors
define $\theta$ (and $d_\theta$). Note that $\psi_\ell: \R^d \to \R^{d_{\ell}}$
and $d_0=d.$ The {\em activation function}
$\sigma: \R \to \R$ is a monotonic non-decreasing function, often
$\sigma(u)={\rm max}(u,0);$ it is extended to a function $\R^s \to \R^s$, 
any integer $s$, elementwise. 


An idealized approach to determining $\theta$ is to minimize the
{\em risk} $$\|\psid-\psi(\cdot;\theta)\|_{\hm}^2.$$
However, this requires knowing $\psid,$ which is of course not given, as well as the pdf $\Upsilon$. 
Instead the optimal parameter $\thetas$ is chosen 
by {\em empirical risk minimization}:
\begin{align}
\label{eq:erm}
\thetas={\rm argmin}_{\theta \in \Theta} \|\psid-\psi(\cdot;\theta)\|_{\hmn}^2.
\end{align}
The {\em empirical risk} is an empirical approximation 
of the  risk $\|\psid-\psi(\cdot;\theta)\|_{\hm}^2$
and only requires knowledge of $\psid$ on the data points
$\{\un\}_{n=1}^N$; this is available to us under the assumption of noiseless data ($\lambda = 0)$ in \eqref{eq:data}.
The empirical risk is typically non-convex as a function of $\theta$, 
with multiple saddle points and local
minima; minimization may be attempted by using stochastic gradient
descent (Chapter \ref{chap:optimization}). 
We write $\psis(u):=\psi(u;\thetas).$

%\subsection{\index{neural network} Neural Networks}\label{ssec:NN}
%A \index{neural network}neural network is a parametric family of functions mapping
%$X$ to $Y$. By use of the data a value of the parameter may be
%chosen so as to determine an approximation of $\psid.$
%To define a \index{neural network}neural network we introduce
%$\Theta \subseteq \R^{d_\theta}$ and then $\psi: \R^d \times \Theta \to \R$
%via the iteration
%\begin{align}
%\label{eq:dnn}
%\psi_0(u;\theta)&=u,\\
%\psi_{\ell+1}(u;\theta)&=\sigma\bigl(W_{\ell}\psi_{\ell}(u)+b_\ell\bigr), \quad
%\ell=0,\dots, L-1,\\
%\psi(u;\theta)&=\beta^\top \psi_{L}(u).
%\end{align}
%In this definition, for $\ell \in \{0,\ldots, L-1\}$,
%$W_{\ell}:\R^{d_{\ell+1}\times d_{\ell}}, b_{\ell} \in \R^{d_{\ell+1}}$
%and $\beta \in \R^{d_{L}};$ together these matrices and vectors
%define $\theta$ (and $d_\theta$). Note that $\psi_\ell: \R^d \to \R^{d_{\ell}}$
%and $d_0=d.$ The {\em activation function}
%$\sigma: \R \to \R$ is a monotonic non-decreasing function, often
%$\sigma(u)={\rm max}(u,0);$ it is extended to a function $\R^s \to \R^s$, 
%any integer $s$, elementwise. 
%
%
%An idealized approach to determining $\theta$ is to minimize the
%{\em risk} $$\|\psid-\psi(\cdot;\theta)\|_{\hm}^2.$$
%However, this requires knowing $\psid$ which is of course not given.
%Instead the optimal parameter $\thetas$ is chosen 
%by {\em empirical risk minimization}:
%\begin{align}
%\label{eq:erm}
%\thetas={\rm argmin}_{\theta \in \Theta} \|\psid-\psi(\cdot;\theta)\|_{\hmn}^2.
%\end{align}
%The {\em empirical risk} is an empirical approximation 
%of the  risk $\|\psid-\psi(\cdot;\theta)\|_{\hm}^2$
%and only requires knowledge of $\psid$ on the data points
%$\{\un\}_{n=1}^N$; this is available to us.
%The empirical risk is typically non-convex as a function of $\theta$, 
%with multiple saddle points and local
%minima; minimization may be attempted by using stochastic gradient
%descent (Chapter \ref{chap:optimization}). 
%We write $\psis(u):=\psi(u;\thetas).$


\subsection{\index{random features}Random Features}\label{ssec:RF}

Now consider a thought experiment in which, rather than optimizing over
all of $\Theta$, the parameters $\ttheta=\{W_{\ell}, b_{\ell}\}_{\ell=0}^{L-1}$
are chosen at random and optimization is performed only over $\beta.$ 
In contrast to full optimization over $\theta,$ this leads to a quadratic optimization problem which is solved by inverting a linear system for $\beta.$ To see this,  note that, if $\varphi_i(u)$ is the $i$-th component of the $\R^{d_L}$--valued function $\psi_{L}$, then
\begin{align}
\label{eq:rf_form}
\psi(u;\beta):=\sum_{i=1}^{d_L}\beta_{i}\varphi_i(u).
\end{align}
Here we view $\psi(\cdot;\beta)$ as parameterized by $\beta$, since
the remaining elements $\ttheta$ of $\theta$ have been picked at 
random and  then fixed. From $\psid$ we may define 
\begin{align}
\label{eq:erm2}
\betas={\rm argmin}_{\beta \in \R^{d_L}} \|\psid-\psi(\cdot;\beta)\|_{\hmn}^2
\end{align}
and $\psis(u):=\psi(u;\betas).$


The collection of functions $\{\varphi_i\}$ are random but
not, in general, \index{i.i.d.}i.i.d.
A variant on this idea is to define $B \subset \R^b$, place
probability measure $q$ on $B$, define functions $\varphi: \R^d \times
B \to \R$ and seek
$$\psi(u;\beta):=\sum_{i=1}^{d_L}\beta_{i}\varphi(u;\ttheta_i), \quad \ttheta_i \sim q, \, \index{i.i.d.}\text{i.i.d.}$$
Empirical risk minimization \eqref{eq:erm2} again leads to a linear system
for $\beta.$ This minimization may be regularized 
and, in place of \eqref{eq:erm2}, $\betas$ is defined via
\begin{align}
\label{eq:erm3}
\betas&={\rm argmin}_{\beta \in \R^{d_L}} \J(\beta),\\
\J(\beta)&:=\frac12\|\psid-\psi(\cdot;\beta)\|_{\hmn}^2+
\frac{\lambda}{2}|\beta|^2.
\end{align}
Again we write $\psis(u):=\psi(u;\betas).$ This regularization may be for instance adequate to deal with noisy data $\xi^{(n)} \sim \mathcal{N}(0, I)$ in \eqref{eq:data} -- see Remark \ref{rem:gpbayes} for a related discussion.

We refer to the functions $\varphi(\cdot;\ttheta)$ as 
{\em random features}\index{random features}.
It is natural to ask how correlated these functions 
are at different points in $D$. To this end, we
introduce a {\em kernel} $c: D \times D \to \R$ defined by
\begin{align}
\label{eq:kernel}
c(u,u'):=\bbE^q \bigl[\varphi(u;\ttheta)\varphi(u';\ttheta) \bigr], 
\end{align}
where expectation is over $\ttheta \sim q.$


\subsection{Gaussian Processes \index{Gaussian!process}}\label{ssec:GP}
The theory of \index{Gaussian!process}Gaussian process regression starts from a kernel 
satisfying two key properties:
\begin{definition}
A kernel $c: D \times D \to \R$ is \emph{symmetric} 
if $c(u,u')=c(u',u)$ for all $(u,u') \in D \times D.$
It is \emph{non-negative definite} if, for all $N \in \mathbb{N},$
all $\{u^{(i)}\}_{i=1}^N  \subset D$ and all $e \in \R^N,$
$$\sum_{i=1}^N \sum_{j=1}^N c\bigl(u^{(i)}, u^{(j)}\bigr) e_i e_j \ge 0.$$ 
If equality implies that $e = 0,$ the kernel is called positive definite. 
\end{definition} 


A symmetric non-negative definite kernel may be viewed as a {\em covariance function}
of a \index{Gaussian}Gaussian random field and we will return to this perspective
at the end of the subsection. 
From non-negative definite, symmetric $c$, we define the integral operator
\begin{align}
\label{eq:IE}
(\cC\phi)(u)=\int_{D} c(u,u')\phi(u') \,du'. 
\end{align}
Provided that $D$ is compact and $c$ is continuous, symmetric and positive 
definite, $\cC$ is a \index{positive definite}positive definite compact operator on $L^2(D)$ and we may define the domain of the inverse of its square root as $K=D(\cC^{-\frac12})$;
furthermore we define 
$K^*$ the dual space of linear functionals on $K$; thus
$K \subset H=L^2(D;\R) \subset K^*$. We assume
that $K^*$ is rich enough that it contains \index{Dirac}Dirac measures in $D$
(and hence pointwise evaluation) and define $\cC^{-1}: K \to K^*.$
It follows that, for all $u' \in D$, 
\begin{align}
\label{eq:GF}
\cC^{-1}c(\cdot,u')=\delta_{u'}(\cdot).
\end{align}

We then seek to define our approximation to $\psid$, function $\psis$,
through the following minimization problem:
\begin{align}
\label{eq:erm4} \psis &={\rm argmin}_{\psi \in K} \J(\psi),\\
\J(\psi)&:=\frac12\|\psid-\psi\|_{\hmn}^2+\frac{\lambda}{2}\|\cC^{-\frac12}\psi\|_{H}^2.
\end{align}
At first sight this appears to be an infinite dimensional optimization problem,
over the whole of $K$. However, it has the following remarkable property, which
is often referred to as the 
{\em representer theorem}\index{representer theorem}, and demonstrates
that the optimization problem is intrinsically finite dimensional: 

\begin{theorem}
Function $\psis$ solving \eqref{eq:erm4} has the form
\begin{align}
\label{eq:eform}
\psis(u)=\sum_{n=1}^N \alphas_n c(u,\un).
\end{align}
Furthermore, the coefficients $\alphas$ solve the
following quadratic minimization problem:
\begin{align}
\label{eq:erm5}
\alphas&={\rm argmin}_{\alpha \in \R^N} \mathsf{A} (\alpha),\\
\mathsf{A}(\alpha)&:=\frac12\Big\|\psid-  \sum_{ n  =1}^N  \alpha_n c(\cdot, \un  )\Big\|_{\hmn}^2+\frac{\lambda}{2}\sum_{n,r=1}^N \alpha_n \alpha_r c(\un,\xr).
\end{align}
\end{theorem}

\begin{proof}
The Euler-Lagrange equations for \index{objective}objective function $\J$ in \eqref{eq:erm4} yield 
$$\lambda (\cC^{-1}\psis)(u)=\frac{1}{N}\sum_{n=1}^N \bigl(\psid(\un)-\psis(\un)\bigr)\delta_{\un}.$$
Now note from \eqref{eq:GF} that $(\cC\delta_{u'})(u)=c(u,u').$ Thus applying
$\cC$ to the Euler-Lagrange equations shows that $\psis(u)$ is in the linear
span of $\{c(\cdot,\un)\}_{n=1}^N,$ establishing the first part of the result.
For the second part, note that
$$\|\cC^{-\frac12}\psi\|_{H}^2=\langle \psi, \cC^{-1} \psi \rangle_{H}.$$
Substituting the established form \eqref{eq:eform}
for $\psis(u)$ into this identity and using \eqref{eq:GF} 
reduces the \index{regularization}regularization term proportional to $\lambda$ to the 
desired form.
\end{proof}

We define $C \in \R^{N \times N}$ to be the matrix with entries
$C_{nr}=c(\un,\xr)$ and $S$ to be its inverse, with entries $S_{nr}$; 
notice that $C$ is positive definite (and hence invertible) provided 
that the kernel $c$ is positive definite. Then we have: 


\begin{corollary}
If $\ps \in \R^N$ is vector with entries $\ps_n=\psis(\un),$ then
$\ps=C\alphas$ and
\begin{align}
\label{eq:erm6}
\ps&={\rm argmin}_{p \in \R^N} \J(p),\\
\J(p)&:=\frac12\sum_{n=1}^N |\psid(\un)-p_n|^2+\frac{\lambda}{2}\sum_{n,r=1}^N p_n p_r S_{n,r}.
\end{align}


\end{corollary}


\begin{remark} \label{rem:gpbayes}
The minimization problem \eqref{eq:erm4} corresponds to determining
the mean of a \index{posterior}posterior distribution of an infinite dimensional \index{Bayesian!inverse problem}Bayesian inverse problem defined as follows. We place as \index{prior}prior on $\psi$ a \index{Gaussian}Gaussian random field with mean zero and covariance function $c(u,u').$  The 
\index{likelihood}likelihood is defined by assuming noisy data in \eqref{eq:data}, 
where $\xi^{(n)} \sim \mathcal{N}(0,I)$ \index{i.i.d.}i.i.d. and then the negative
\index{posterior}log-posterior density is given by $\lambda^{-1}\J(\psi).$  
The \index{posterior}posterior mean, which is also a form of \index{MAP estimator}MAP estimator, 
then satisfies \eqref{eq:erm4}. We also remark that minimization 
of \eqref{eq:erm3} also has a similar interpretation as a \index{MAP estimator}MAP
estimator, but with respect to a \index{Gaussian!process}Gaussian process with  mean zero and covariance function a random approximation
of $c(u,u').$ 
\end{remark}
 

%\subsection{Gaussian Processes \index{Gaussian!process}}\label{ssec:GP}
%
%\as Conditions on kernel to make operator compact etc. \nc
%
%
%%Recall the support $D$ of probability measure $\mu$, noting that the
%%training data $\{x_n\}_{n=1}^N \subset D.$
%The theory of \index{Gaussian!process}Gaussian process regression starts from a kernel 
%satisfying two key properties:
%\begin{definition}
%A kernel $c: D \times D \to \R$ is \emph{symmetric} 
%if $c(u,u')=c(u',u)$ for all $(u,u') \in D \times D.$
%It is \emph{non-negative definite} if, for all $N \in \mathbb{N},$
%all $\{u^{(i)}\}_{i=1}^N$ in $\R^N$ and all $e \in \R^N$
%$$\sum_{i=1}^N \sum_{j=1}^N c\bigl(u^{(i)}, u^{(j)}\bigr) e_i e_j \ge 0.$$ 
%\end{definition} 
%
%
%
%This may be viewed as a {\em covariance function}
%of a \index{Gaussian}Gaussian random field and we will return to this perspective
%at the end of the subsection. 
%From non-negative definite, symmetric $c$, we define the integral operator
%\begin{align}
%\label{eq:IE}
%(\cC\phi)(u)=\int_{D} c(u,u')\phi(u') \,du'.
%\end{align}
%This is a \index{positive definite}positive definite compact operator on $L^2(D)$ and we may define the domain of the inverse of its square root as $K=D(\cC^{-\frac12})$;
%furthermore we define 
%$K^*$ the dual space of linear functionals on $K$; thus
%$K \subset H=L^2(D;\R) \subset K^*$. We assume
%that $K^*$ is rich enough that it contains \index{Dirac}Dirac measures in $D$
%(and hence pointwise evaluation) and define $\cC^{-1}: K \to K^*.$
%It follows that
%\begin{align}
%\label{eq:GF}
%\cC^{-1}c(\cdot,u')=\delta_{u'}(\cdot).
%\end{align}
%
%We then seek to define our approximation to $\psid$, function $\psis$,
%through the following minimization problem:
%\begin{align}
%\label{eq:erm4} \psis &={\rm argmin}_{\psi \in K} \J(\psi),\\
%\J(\psi)&:=\frac12\|\psid-\psi\|_{\hmn}^2+\frac{\lambda}{2}\|\cC^{-\frac12}\psi\|_{H}^2.
%\end{align}
%At first sight this appears to be an infinite dimensional optimization problem,
%over the whole of $K$. However it has the following remarkable property, which
%is often referred to as the 
%{\em representer theorem}\index{representer theorem}:
%
%\begin{theorem}
%Function $\psis$ solving \eqref{eq:erm4} has the form
%\begin{align}
%\label{eq:eform}
%\psis(u)=\sum_{n=1}^N \alphas_n c(u,\un).
%\end{align}
%Furthermore, the coefficients $\alphas$ solve the
%following quadratic minimization problem:
%\begin{align}
%\label{eq:erm5}
%\alphas&={\rm argmin}_{\alpha \in \R^N} \J(\alpha),\\
%\J(\alpha)&:=\frac12\Big\|\psid-\sum_{r=1}^N \alpha_n c(\cdot,\xr)\Big\|_{\hmn}^2+\frac{\lambda}{2}\sum_{n,r=1}^N \alpha_n \alpha_r c(\un,\xr).
%\end{align}
%\end{theorem}
%
%\begin{proof}
%The Euler-Lagrange equations for \index{objective}objective function $\J$ yield \ds conflict two objectives $\J.$ \nc
%$$\lambda (\cC^{-1}\psis)(u)=\frac{1}{N}\sum_{n=1}^N \bigl(\psid(\un)-\psis(\un)\bigr)\delta_{\un}.$$
%Now note from \eqref{eq:GF} that $(\cC\delta_{u'})(u)=c(u,u').$ Thus applying
%$\cC$ to the Euler-Lagrange equations shows that $\psis(u)$ is in the linear
%span of $\{c(\cdot,\un)\}_{n=1}^N,$ establishing the first part of the result.
%For the second part, note that
%$$\|\cC^{-\frac12}\psi\|_{H}^2=\langle \psi, \cC^{-1} \psi \rangle_{H}.$$
%Substituting the established form \eqref{eq:eform}
%for $\psis(u)$ into this identity and using \eqref{eq:GF} 
%reduces the \index{regularization}regularization term proportional to $\lambda$ to the 
%desired form.
%\end{proof}
%
%We define $C \in \R^{N \times N}$ to be the matrix with entries
%$C_{nr}=c(\un,\xr)$ and $S$ to be its inverse, with entries $S_{nr}$,
%then we have: 
%
%
%\begin{corollary}
%If $\ps \in \R^N$ is vector with entries $\ps_n=\psis(\un),$ then
%$\ps=C\alphas$ and
%\begin{align}
%\label{eq:erm6}
%\ps&={\rm argmin}_{p \in \R^N} \J(p),\\
%\J(p)&:=\frac12\sum_{n=1}^N |\psid(\un)-p_n|^2+\frac{\lambda}{2}\sum_{n,r=1}^N p_n p_r S_{n,r}.
%\end{align}
%
%
%\end{corollary}
%
%
%\begin{remark} \label{rem:gpbayes}
%The minimization problem \eqref{eq:erm4} corresponds to determining
%the mean of a \index{posterior}posterior distribution of an infinite dimensional \index{Bayesian!inverse problem}Bayesian inverse problem defined as follows. We place as \index{prior}prior on $\psi$ a \index{Gaussian}Gaussian random field with mean zero and covariance function $c(u,u').$  The 
%\index{likelihood}likelihood is defined by assuming \eqref{eq:review}, 
%where $\xi^{(n)} \sim \mathcal{N}(0,I)$ \index{i.i.d.}i.i.d. and then the negative
%\index{posterior}log-posterior density is given by $\lambda^{-1}\J(\psi).$  
%The \index{posterior}posterior mean, which is also a form of \index{MAP estimator}MAP estimator, 
%then satisfies \eqref{eq:erm4}. We also remark that minimization 
%of \eqref{eq:erm3} also has a similar interpretation as a \index{MAP estimator}MAP
%estimator, but with respect to a \index{Gaussian!process}Gaussian process with  mean zero and covariance function a random approximation
%of $c(u,u').$ 
%\end{remark}


\subsection{Approximation Properties}
\label{ssec:AP}
All of the preceding three methods can, in principle, approximate
continuous functions to arbitrary accuracy, over a compact set.
Doing so requires sufficient data. Furthermore, in the case of 
\index{neural network}neural networks, this also requires sophisticated optimization 
techniques to obtain close to optimal solutions; in contrast,
the \index{random features}random features and \index{Gaussian!process}Gaussian process approaches only require solution
of linear systems, resulting from a quadratic optimization problem.
Typical instances of the resulting approximation theory for
the three supervised learning techniques typically shows that, 
for given $\delta>0$, 
there is a volume of data $N$ such that, with high probability with
respect to the data,
\begin{equation}
\label{eq:eb}
\sup_{u \in D} |\psid(u)-\psi^\star(u)| < \delta.
\end{equation}
Theory establishing results of this form is cited in the bibliography
Section \ref{sec:IPMLBib}.


\section{\index{transport!measure} \index{unsupervised learning}Unsupervised Learning}
\label{sec:MT}
 In this subsection we study a part of the methodology of
\index{unsupervised learning}unsupervised learning which is
often referred to as \emph{generative modeling}\index{generative model}. 
We start by discussing the {\em measure transport} task of determining
function $g: \R^{\dz} \to \R^d$ so that, given 
pdf $\zeta$ on $\R^{\dz}$ and pdf $\Upsilon$ on $\R^d$,
$g^\sharp \zeta = \Upsilon;$ here $g^\sharp$ denotes the 
pushforward\index{pushforward}  operation
and so, explicitly, we are seeking $g$ so that, if $z \sim \zeta$, then
$g(z) \sim \Upsilon.$ An important area of \index{machine learning}machine learning where this
arises is in the \index{unsupervised learning}{\em unsupervised learning} problem as follows.  
We have available to us data in the form
\begin{align}
\label{eq:datau}
\{\un\}_{n=1}^N,
\end{align}
assumed to be drawn \index{i.i.d.}i.i.d. from pdf $\Upsilon$ which is unknown to us. Hence we have access to the empirical density 
\begin{align}
\label{eq:emp}
\mn(u)=\frac{1}{N} \sum_{n=1}^N \delta(u-\un).
\end{align}

In \index{unsupervised learning}unsupervised learning the goal is to understand the data set
summarized by measure $\mn.$ One approach is to study
{\em clustering}\index{clustering} within the data; we will not
pursue this important topic because it is not of direct relevance
to the solution of \index{inverse problem}inverse problems, our focus in these notes.
Instead we pursue the approach of \index{generative model}{\em generative modeling}.
Assume that $\zeta$ is \index{Gaussian}Gaussian, then the aim 
is to find map $g$ so that samples
from \index{Gaussian}Gaussian $\zeta$, when pushed forward under $g$, will look like
samples from $\Upsilon$. 
We will also study relaxations of this problem, in which the
\index{Gaussian}Gaussian $\zeta$ is convolved with a \index{Gaussian}Gaussian whose mean is function $g$.


As for \index{supervised learning}supervised learning, the task of identifying
$g$ in the models described above must be undertaken empirically, since only $\mn$ is available to us, not $\Upsilon.$

\subsection{\index{transport!optimal} Optimal Transport Maps}\label{ssec:OPT}

 Although optimal transport\index{transport!optimal} does not lead to 
algorithms for inverse problems used in this chapter, it plays an
important underpinning role in the theory of measure transport, which does
play a role in the algorithms used in this chapter. 
Given the two densities $\zeta,\Upsilon$ on $\R^{\dz}, \R^d$ respectively, we define a \index{coupling}{\em coupling} as a density $\pi$ on $\R^{\dz} \times \R^d$ with the property that
$$\int_{\R^d} \pi(z,u) \, du=\zeta(z), \quad \int_{\R^{\dz}} \pi(z,u) \, dz=\Upsilon(u).$$
Thus the marginals of $\pi$ deliver $\zeta$ and $\Upsilon$.
We denote the set of all such \index{coupling}couplings by $\Pi_{\zeta,\Upsilon}.$
Given a cost function $\co: \R^{\dz} \times \R^d \to \R^+$ we
define the Kantorovich formulation of the 
optimal transport \index{optimal transport!Kantorovich}
problem as follows:
\begin{align}
\label{eq:KOT}
\pist&={\rm arginf}_{\pi \in \Pi_{\zeta,\Upsilon}} 
\int_{\R^{\dz} \times \R^d} \co(z,u)\pi(z,u) \, dz du.
\end{align}

This notion of \index{optimal transport}optimal transport may be used to define
families of metrics on probability densities as follows.
If $\dz =d$, so that $\zeta, \Upsilon$ are both densities 
on the same space $\R^d$, then given a metric $\dm(\cdot,\cdot)$
on $\R^d$ and an integer $p$, we define
\begin{align}
\label{eq:WP}
W_{p}(\zeta,\Upsilon)&=\Bigl({\rm inf}_{\pi \in \Pi_{\zeta,\Upsilon}}
\int_{\R^{\dz} \times \R^d} \dm(z,u)^p\pi(z,u) \,dz du\Bigr)^{\frac{1}{p}}.
\end{align}
This metric on probability measures has two key aspects:
first, it relates the metric to an underlying metric on
$\R^d$; and second, it allows for a meaningful \index{distance}distance to
be calculated between measures which are mutually singular. It is known as a Wasserstein$-p$ 
distance\index{distance!Wasserstein}. 

\begin{example}
Let $p_i=\cN(m_i,\Sigma_i)$ for $i=1,2.$ 
It may be shown that, if the metric $\dm$ induced by the Euclidean
norm $|\cdot|$ is used, then
$$W_{2}(p_1,p_2)^2= |m_1-m_2 |^2+{\rm Tr}\Bigl(\Sigma_1+\Sigma_2-
2\bigl(\Sigma_1^{\frac12}\Sigma_2 \Sigma_1^{\frac12}\bigr)\Bigr).$$
In particular, if $p_2$ is a \index{Dirac}Dirac measure at the origin then
$$W_{2}(p_1,p_2)^2= |m_1 |^2+{\rm Tr}\bigl(\Sigma_1\bigr).$$

Thus, in the \index{distance!Wasserstein}Wasserstein$-2$ metric \index{Gaussian}Gaussian $p_1$ is close to
a \index{Dirac}Dirac at the origin if the mean and covariance of $p_1$ are
both small. 
In contrast, the total variation 
distance\index{distance!total variation}
between Gaussian $p_1$ and a Dirac at the origin is maximal, and equal to $1$, 
unless
the two measures coincide ($m_1=0, \Sigma_1=0$) when it is $0.$
Similarly the \index{divergence!Kullback-Leibler}Kullback-Leibler divergence becomes infinite as $p_2$
approaches a \index{Dirac}Dirac limit, from within the class of \index{Gaussian}Gaussians -- see
Example \ref{ex:klg}. 


Notice also that if $p_1$ and $p_2$ are \index{dirac}Diracs at $m_1$ and $m_2$, then $W_2(p_1,p_2) = |m_1 - m_2|;$ thus closeness in the location of the mass locations $m_1$ and $m_2$ in Euclidean space translates into closeness of $p_1$ and $p_2$ in \index{distance!Wasserstein}Wasserstein distance. 
\end{example} 

The connection of \index{optimal transport}optimal transport to explicit transport maps
is made clear in the Monge formulation of optimal 
transport\index{optimal transport!Monge}. In this formulation
we explicitly link $\Upsilon$ with a pushforward\index{pushforward} of $\zeta$ and identify the
pushforward map which minimizes the cost:
\begin{align}
\label{eq:KOT}
\gs&={\rm arginf}_{g: g^\sharp \zeta = \Upsilon}
\int_{\R^{\dz}} \co\bigl(z,g(z)\bigr) \zeta(z)\, dz.
\end{align}
Under certain smoothness assumptions, the Kantorovich formulation
has solution within the Monge class. That is, the optimal \index{coupling}coupling is
constructed using the pushforward\index{pushforward}: 
$$\pist(z,u)=\delta\bigl(u-{\gs(z)}\bigr) \zeta(z).$$

Whilst \index{optimal transport}optimal transport provides a deep mathematical structure within
which to consider the \index{transport!measure}measure transport problem, there are numerous
applications where the optimality constraint on the transport confers
few advantages over other transports. Furthermore, it makes the computational task of finding the transport quite difficult. For these reasons a number of other approaches to transport have been considered and we discuss some of them in the remaining subsections of this section. 




%\subsection{\index{transport!optimal} Optimal Transport Maps}\label{ssec:OPT}
%Given the two densities $\zeta,\Upsilon$ on $\R^{\dz}, \R^d$ respectively, we define a \index{coupling}{\em coupling} as a density $\pi$ on $\R^{\dz} \times \R^d$ with the property that
%$$\int_{\R^d} \pi(z,u) \, du=\zeta(z), \quad \int_{\R^{\dz}} \pi(z,u) \, dz=\Upsilon(u).$$
%Thus the marginals of $\pi$ deliver $\zeta$ and $\Upsilon$.
%We denote the set of all such \index{coupling}couplings by $\Pi_{\zeta,\Upsilon}.$
%Given a cost function $\co: \R^{\dz} \times \R^d \to \R^+$ we
%define the Kantorovich formulation of the 
%optimal transport \index{optimal transport!Kantorovich}
%problem as follows:
%\begin{align}
%\label{eq:KOT}
%\pist&={\rm arginf}_{\pi \in \Pi_{\zeta,\Upsilon}} 
%\int_{\R^{\dz} \times \R^d} \co(z,u)\pi(z,u) \, dz du.
%\end{align}
%
%This notion of \index{optimal transport}optimal transport may be used to define
%families of metrics on probability densities as follows.
%If $\dz =d$, so that $\zeta, \Upsilon$ are both densities 
%on the same space $\R^d$, then given a metric $\dm(\cdot,\cdot)$
%on $\R^d$ and an integer $p$, we define
%\begin{align}
%\label{eq:WP}
%W_{p}(\zeta,\Upsilon)&=\Bigl({\rm inf}_{\pi \in \Pi_{\zeta,\Upsilon}}
%\int_{\R^{\ds \dz \nc} \times \R^d} \dm(z,u)^p\pi(z,u) \,dz du\Bigr)^{\ds \frac{1}{p} \nc}.
%\end{align}
%This metric on probability measures has two key aspects:
%first, it relates the metric to an underlying metric on
%$\R^d$; and second, it allows for a meaningful \index{distance}distance to
%be calculated between measures which are mutually singular. It is known as a Wasserstein$-p$ 
%distance\index{distance!Wasserstein}. 
%
%\begin{example}
%Let $p_i=\cN(m_i,\Sigma_i)$ for $i=1,2.$ 
%It may be shown that, if the metric $\dm$ induced by the Euclidean
%norm $|\cdot|$ is used, then
%$$W_{2}(p_1,p_2)^2= |m_1-m_2 |^2+{\rm Tr}\Bigl(\Sigma_1+\Sigma_2-
%2\bigl(\Sigma_1^{\frac12}\Sigma_2 \Sigma_1^{\frac12}\bigr)\Bigr).$$
%In particular, if $p_2$ is a \index{Dirac}Dirac measure at the origin then
%$$W_{2}(p_1,p_2)^2= |m_1 |^2+{\rm Tr}\bigl(\Sigma_1\bigr).$$
%Thus, in the \index{distance!Wasserstein}Wasserstein$-2$ metric \index{Gaussian}Gaussian $p_1$ is close to
%a \index{Dirac}Dirac at the origin if the mean and covariance of $p_1$ are
%both small. In contrast, the total variation 
%distance\index{distance!total variation}
%between $\mu$ and $\nu$ is maximal, and equal to $1$, unless
%the two measures coincide ($m_1=0, \Sigma_1=0$) when it is $0.$
%Similarly the \index{divergence!Kullback-Leibler}Kullback-Leibler divergence becomes infinite as $p_2$
%approaches a \index{Dirac}Dirac limit, from within the class of \index{Gaussian}Gaussians -- see
%Example \ref{ex:klg}. \ds Notice also that if $p_1$ and $p_2$ are \index{dirac}Diracs at $m_1$ and $m_2$, then $W_2(p_1,p_2) = |m_1 - m_2|;$ thus closeness in the location of the mass locations $m_1$ and $m_2$ in Euclidean space translates into closeness of $p_1$ and $p_2$ in \index{distance!Wasserstein}Wasserstein distance. \nc
%\end{example} 
%
%The connection of \index{optimal transport}optimal transport to explicit transport maps
%is made clear in the Monge formulation of optimal 
%transport\index{optimal transport!Monge}. In this formulation
%we explicitly link $\Upsilon$ with a pushforward\index{pushforward} of $\zeta$ and identify the
%pushforward map which minimizes the cost:
%\begin{align}
%\label{eq:KOT}
%\gs&={\rm arginf}_{g: g^\sharp \zeta = \Upsilon}
%\int_{\R^{\ds \dz \nc}} \co\bigl(z,g(z)\bigr) \zeta(z)\, dz.
%\end{align}
%Under certain smoothness assumptions the Kantorovich formulation
%has solution within the Monge class, that is the optimal \index{coupling}coupling is
%constructed using the pushforward: 
%$$\pist(z,u)=\delta\bigl(u-{\gs(z)}\bigr) \zeta(z).$$
%
%Whilst \index{optimal transport}optimal transport provides a deep mathematical structure within
%which to consider the \index{transport!measure}measure transport problem, there are numerous
%applications where the optimality constraint on the transport confers
%few advantages over other transports. Furthermore, it makes the computational task of finding the transport quite difficult. For these reasons a number of other approaches to transport have been considered and we discuss some of them in the remaining subsections of this section. 

\subsection{Other Transport Approaches}\label{ssec:transport2}
\index{transport}
Let $\pi, \pi'$ be two pdfs on $\R^d$. 
We consider the task of finding invertible 
$g: \R^d \to \R^d$ with the property that $\pi \approx g^\sharp \pi'$;
equivalently, since $g$ is invertible, $\pi' \approx (g^{-1})^\sharp \pi.$
We seek to determine a parameter such that $g$ chosen from the parametric class $g: \R^d \times \Theta_g \mapsto \R^d$, with 
$\Theta_g \subseteq \R^{p_g},$ realizes this approximation.
To this end we define
$$F(\theta_g)=\dkl \bigr(\pi \| g(\cdot; \theta_g)^\sharp \pi' \bigl)$$
and set
$$\thetas_g={\rm argmin}_{\theta_g \in \Theta_g} F(\theta_g).$$
We define the resulting approximate pushforward\index{pushforward} map by $\gs=g(\cdot;\thetas_g).$
Note that there exist perfect transport functions $g_{\rm perfect}$
(for example an \index{optimal transport}optimal transport)
for which $\dkl(\pi \| g_{\rm perfect}^\sharp \pi')=0$. We aim
to get as close as possible to such solutions, within our
parametric class, by minimizing $F$ over $\theta_g.$

The following lemma is useful in determining an explicit form
of $F$ for computational purposes.
The proof is a straightforward consequence of change of variables.

\begin{lemma}
\label{lem:cov}
Let $\pi'$ be a probability density on $\R^d$ and
let $\ff \in C^1(\R^d,\R^d)$ be invertible everywhere on $\R^d$. 
Assume further that the determinant of the Jacobian of the inverse, 
\begin{equation*}
{\rm det} D(\ff^{-1})(u)=\Bigl({\rm det} D\ff\bigl(\ff^{-1}(u)\bigr)\Bigr)^{-1},
\end{equation*}
is positive everywhere on $\R^d$. Then, for $u=q(z)$,
$$\int_{\R^d} \phi(z)\pi'(z) \, dz=\int_{\R^d} \bigl(\phi \circ \ff^{-1}\bigr)(u)
\bigl(\pi' \circ \ff^{-1}\bigr)(u) {\rm det} D(\ff^{-1})(u) \, du .$$
Thus 
$$\ff^\sharp \pi'(u)= \bigl(\pi' \circ \ff^{-1}\bigr)(u) {\rm det} D(\ff^{-1})(u).$$
\begin{equation}
\label{eq:cov}
\log \ff^\sharp \pi'(u) = \log \bigl(\pi' \circ \ff^{-1}\bigr)(u) -
 \log {\rm det} D\ff\bigl(\ff^{-1}(u)\bigr). 
\end{equation}
\end{lemma} 

Using the expression for the density of the pushforward\index{pushforward} we find that, for differentiable $g$, 
\begin{subequations}
\label{eq:OT}
\begin{align}
F(\theta_g) & = \bbE^{u \sim \pi} \Bigl[\log \pi(u) - \log g^\sharp \pi'(u)\Bigr]\\
& =  -\bbE^{u \sim \pi} \Bigl[\log \pi' \circ g^{-1}(u;\theta_g)+ \log {\rm det}  D_u(g^{-1})(u;\theta_g) \Bigr]+{\rm const},
\end{align}
\end{subequations}
where the constant term is independent of $g$, and hence of $\theta_g;$
it can be ignored for the purposes of minimization.
Note also that, using \eqref{eq:cov}, 
and neglecting the constant term, we may also write
\begin{equation}
\label{eq:OT99}
F(\theta_g)= -\bbE^{u \sim \pi} \Bigl[\log \pi' \circ g^{-1}(u;\theta_g)- \log {\rm det}  D_u g\bigl(g^{-1}(u;\theta_g);\theta_g\bigr) \Bigr].
\end{equation}

\begin{remark}
\label{rem:discuss}
This approach can be implemented in the setting where $\pi=\Upsilon$
and $\pi'=\zeta$, detailed at the start of the section. In this setting
$\pi=\Upsilon$ is only available empirically. 
Since $F$ is defined as an expectation over $\pi$, this is
readily approximated empirically. We thus find an approximate
expression for $\pi$, known only through samples,
as the image under $\gs$ of $\pi'.$ 
Once we have the map $\gs$ we can generate new (approximate)
samples from $\pi$ by \index{sampling}sampling $\pi'$ and applying $\gs.$
An important issue here is that we are interested in determining
the optimal \index{forward!map}forward map $g$, but the optimization problem, for either
choice of $F(\theta_g)$ in \eqref{eq:OT} or \eqref{eq:OT99}, 
necessarily involves $g^{-1}.$ Thus $g$ must be readily invertible. 
Subsection \ref{ssec:NORM} addresses this issue in the context 
of \index{normalizing flow}normalizing flows.



We have introduced $\pi$ and $\pi'$, rather than working with
$\Upsilon$ and $\zeta$ from the outset, because the approach as outlined
is useful in a different setting in Section \ref{sec:LPrtoPo}.
In Section \ref{sec:LPrtoPo} $\pi$ is typically a known simple measure, from
which samples are easily drawn, whereas $\pi'$ is a more
complicated measure which we wish to characterize and sample
from; in such a setting, the objective is to determine $T=g^{-1}$
so that $\pi'=(g^{-1})^\sharp \pi.$ Since \eqref{eq:OT} is expressed
entirely in terms of $T=g^{-1}$, and not $g$ itself, it is possible
to approach this problem by directly parameterizing $T=g^{-1}$ rather
than $g.$ 
\end{remark}



\subsection{Autoencoders\index{autoencoder}}\label{ssec:auto}
Autoencoders are primarily used as a technique for uncovering
latent low-dimensional structure in high dimensional data. We introduce
them here and then demonstrate in the next subsection that a natural
probabilistic relaxation of the idea leads to generative models 
termed \index{variational!autoencoder}\index{autoencoder!variational}variational autoencoders.

\index{transport}Transport ideas may be used to (approximately) represent a complicated 
probability distribution, perhaps only known through samples, as the 
pushforward\index{pushforward} of a simpler measure. In this section we go a step further,
by seeking a simpler measure which lives in a lower dimensional \index{latent}latent space.
\index{autoencoder}Autoencoders are one natural approach to such problems.

The basic idea of \index{autoencoder}autoencoders is to find an approximate factorization
of the identity which is accurate in the support of density $\Upsilon$, but
using only the empirical approximation of $\Upsilon$ by $\mn$. 
Let $f: \R^d \times \Theta_f \mapsto \R^{\dz}$
and  $g: \R^{\dz} \times \Theta_g \mapsto \R^d$ where $\Theta_f \subseteq
\R^{p_f}$ and $\Theta_g \subseteq \R^{p_g};$ in particular each of $f$
and $g$ can be a \index{neural network}neural network, as defined in Subsection \ref{ssec:NN},
generalized to vector-valued output. Recalling that $Id$ denotes the 
identity mapping on $\R^d$, and defining 
$$F(\thetas_f,\thetas_g)= 
\Bigl\|Id-g\bigl(f(\cdot;\theta_f);\theta_g\bigr)\Bigr\|_{\hm}^2$$ 
we consider the following optimization problem: 
\begin{align} 
\label{eq:erm99} 
(\thetas_f,\thetas_g)={\rm argmin}_{(\theta_f,\theta_g) \in \Theta_f \times
\Theta_g} F(\thetas_f,\thetas_g). 
\end{align}
We then define $\fs(u)=f(u,\thetas_f)$ and $\gs(z)=g(z,\thetas_g).$
Roughly speaking, and dropping the dependence on parameters for
expository purposes, we are seeking functions $f$ and $g$ 
such that $g\bigl(f(u)\bigr) \approx u.$ In practice the
optimization is implemented empirically, and the norm on $\hm$ in $F$
is replaced by the norm on $\hmn.$


This approach reduces the \index{autoencoder}autoencoder to a particular form of supervised
learning in which the inputs and outputs are equal, so we seek to
approximate the identity, and in which we impose
a specific structure on the class of approximating function -- as
composition of $g$ with $f$. 
We refer to $\R^{\dz}$ as the {\em latent space}\index{latent}
and note that a primary application of the methodology 
is to identify \index{latent}latent spaces of dimension
$\dz$ which is much less than the dimension $d$ of the data space. The
approximate factorization of the identity found by composing $g$ with $f$
provides a way of moving between the data space and the \index{latent}latent space.

\subsection{Variational Autoencoders \index{variational!autoencoder}\index{autoencoder!variational}}\label{ssec:vauto}
In the preceding subsection, note that $\zeta=(\fs)^\sharp \Upsilon$ 
gives the (approximate) distribution 
in the \index{latent}latent space, but that we cannot specify $\zeta$; mapping
$g$ (approximately) solves a \index{transport!measure}measure transport problem from $\zeta$ to $\Upsilon$, 
but choice of measure $\zeta$ is not within our control. 
It is natural to ask whether the methodology can be 
generalized to settings in which it is desirable
to impose a specified distribution $\zeta$. This leads to the topic
of {\em variational autoencoders.} \index{variational!autoencoder}\index{autoencoder!variational}

To this end let $\pi$ be a \index{coupling}coupling of $\Upsilon$ and $\zeta$ 
and note that the following two identities hold:
\begin{align*}
\pi(u,z)&=\bbP(u|z)\zeta(z),\\
\pi(u,z)&=\bbP(z|u)\Upsilon(u).
\end{align*}
The idea of the \index{variational!autoencoder}\index{autoencoder!variational}variational autoencoder is to approximate the two conditional
densities $\bbP(u|z), \bbP(z|u)$ appearing in these identities by 
parameterized families. A parametric choice is made to ensure that the two  
resulting approximate expressions for $\pi(u,z)$ are close. 
To be explicit we assume that
\begin{align*}
u|z & \sim \cN\bigl(g(z;\theta_g),\sigma_g^2 I\bigr),\\
z|u & \sim \cN\bigl(f(u;\theta_f),\sigma_f^2 I\bigr), 
\end{align*}
noting that this is a relaxation of the setting for \index{autoencoder}autoencoders.
Invoking these \index{Gaussian!approximation}Gaussian approximations for the conditionals we obtain
the following two approximations for the \index{coupling}coupling density:
\begin{align*}
\pi_g(u,z)&=\frac{1}{Z_g}\exp\Bigl(-\frac{1}{2\sigma_g^2}|u-g(z;\theta_g)|^2\Bigr) \zeta(z),\\
\pi_f(u,z)&=\frac{1}{Z_f}\exp\Bigl(-\frac{1}{2\sigma_f^2}|z-f(u;\theta_f)|^2\Bigr) \Upsilon(u).
\end{align*}
A common choice is to assume that $\zeta$ is the density of
a standard unit \index{Gaussian}Gaussian; we make this assumption throughout what follows.

For simplicity,  we consider the standard deviations 
$\sigma_f, \sigma_g$ to be fixed, and determine the parameters 
of $f$ and $g$.  We do this by asking that $\pi_f$ and
$\pi_g$ are close. If we measure closeness by means of 
\index{divergence!Kullback-Leibler}Kullback-Leibler divergence, with $\pi_f$ in the first argument,
then using the \index{Gaussian}Gaussian assumptions on the conditionals and on $\zeta$
leads to insightful explicit calculations. To see this, we first note that 
\begin{align*}
\dkl(\pi_f\|\pi_g) = \bbE^{u \sim \Upsilon} \biggl[\bbE^{z \sim \bbP(z|u)}
%\cN\bigl(f(u;\theta_f),\sigma_f^2 I\bigr)}
\Bigl[ \frac{1}{2\sigma_g^2}|u-g(z;\theta_g)|^2 \Bigr] +
\dkl\bigl(\bbP(\cdot|u)\| \zeta \bigr)\biggr]+{\rm const},
\end{align*}
where the constant is independent of the parameters we wish to learn
and where $\bbP(z|u)$ and $\zeta(z)$ are given by their assumed \index{Gaussian}Gaussian structure.
Using the expression in Example \ref{ex:klg} for the \index{divergence!Kullback-Leibler}Kullback-Leibler
divergence between two \index{Gaussian}Gaussians we obtain
\begin{align*}
\dkl(\pi_f\|\pi_g) = \bbE^{u \sim \Upsilon} \biggl[\bbE^{z \sim \cN\bigl(f(u;\theta_f),\sigma_f^2 I\bigr)} \Bigl[\frac{1}{2\sigma_g^2}\big|u-g(z;\theta_g)\big|^2 \Bigr]+
\frac{1}{2}|f(u;\theta_f)|^2\biggr]+{\rm const.}
\end{align*}
Noting that, $z \sim \cN\bigl(f(u;\theta_f),\sigma_f^2 I\bigr)$ is
the same in law as $f(u;\theta_f)+\sigma_f \xi$ where $\xi \sim
\cN(0,I)$ we may write this \index{divergence}divergence as
\begin{align*}
\dkl(\pi_f\|\pi_g) = 
F(\theta_f,\theta_g)+{\rm const.}
\end{align*} 
where
\begin{align*}
F(\theta_f,\theta_g) = \bbE^{u \sim \Upsilon} \biggl[\bbE^{\xi \sim \cN(0,I)} \Bigl[\frac{1}{2\sigma_g^2}\Big|u-g\bigl(f(u;\theta_f)+\sigma_f \xi;\theta_g\big)\Big|^2 \Bigr]+
\frac{1}{2}|f(u;\theta_f)|^2\biggr]
\end{align*}
and the constant term is independent of $(\theta_f,\theta_g).$


This constitutes a regularized version of the standard \index{autoencoder}autoencoder;
in particular the preceding expression for the \index{divergence}divergence clearly
regularizes the basic concept that $g\bigl(f(u)\bigr) \approx u$
under density $\Upsilon.$ 


\begin{remark}
In practice this is implemented with expectation 
over $\Upsilon$ approximated empirically by $\mn.$
This leaves an optimization problem in which the \index{objective}objective
is defined via expectation over $\xi.$ Stochastic
gradient descent\index{gradient descent!stochastic} from
Chapter \ref{chap:optimization} 
may be used to tackle this problem. After training, approximate samples 
from $\Upsilon$ may be obtained by sampling $z\sim \zeta$ and then 
sampling $u|z \sim \Nc \bigl(g(z; \theta_g), \sigma_g^2\big)$. 
\end{remark}

\subsection{Generative Adversarial Networks}\label{ssec:gan}
\index{generative adversarial network}


The \index{variational!autoencoder}\index{autoencoder!variational}variational autoencoder trains a probabilistic model
for $u$, by learning $\bbP(u|z)$ and specifying $\bbP(z).$
The \index{generative adversarial network}generative adversarial network is
another method for training such a probabilistic model, which
also allows for low dimensional \index{latent}latent space. 
To be concrete we assume that it has the same structural 
form, namely
\begin{align*}
u|z & \sim \cN\bigl(g(z;\theta_g),\sigma_g^2 I\bigr),\\
z & \sim \cN\bigl(0,I\bigr).
\end{align*}
Thus samples from $u$ are created from samples from $z$. We
write the resulting density of $u$ as $\Upsilon_g$, with $g$ for generative. 
It is desired that samples from $\Upsilon_g$ are similar to those
specified by the data, which is drawn from density $\Upsilon$.

The \index{generative adversarial network}generative adversarial network starts by defining a
\emph{discriminator} $\mathsf{d}: \R^d \times \Theta_{\mathsf{d}} \to [0,1]$,
to be thought of as taking values which are probabilities.
Here $\Theta_{\mathsf{d}} \subset \bbR^{p_{\mathsf{d}}}.$ 
It is instructive to think of $\mathsf{d}(u;\theta_{\mathsf{d}})$ as being the
probability that $u$ is drawn from the density $\Upsilon$, and
$1- \mathsf{d} (u;\theta_{ \mathsf{d} })$ as the probability of $u$ being drawn
from the \index{generative model}generative model $\Upsilon_g.$
We then define $v: \Theta_g \times \Theta_{ \mathsf{d} } \to \bbR$ by
$$v(\theta_g,\theta_{ \mathsf{d} })=\bbE^{u \sim \Upsilon} \bigl[\log  \mathsf{d}  (u; \theta_{ \mathsf{d} }) \bigr] +
\bbE^{u \sim \Upsilon_g} \bigl[\log \bigl(1-  \mathsf{d}  (u; \theta_{ \mathsf{d} })\bigr)\bigr].$$
The optimal parameter values are defined by
\begin{align*}
\theta'_{ \mathsf{d} }(\theta_g) & = {\rm argmax}_{\theta_{ \mathsf{d} }} v(\theta_g,\theta_{ \mathsf{d} }),\\
\thetas_g & ={\rm argmin}_{\theta_g} v\bigl(\theta_g,\theta'_{ \mathsf{d} }(\theta_g)\bigr),\\
\thetas_{ \mathsf{d}} & = \theta'_{ \mathsf{d} }(\thetas_g).
\end{align*}
In the maximization step, the parameters of the discriminator are chosen
to maximize $v$ -- the discriminator acts adversarially to try and find data
under $\Upsilon_g$ which does not look like data under $\Upsilon$. In the minimization
step the generator acts to reduce $v$ to try and make the two data sources
look similar. Ideally, through an iterative process, a solution is found in
which $ \mathsf{d}  (\cdot;\thetas_{ \mathsf{d} }) \equiv \frac12$, so that the data and generated
data are indistinguishable. The value of $\thetas_g$ defines the generative
model once this indistinguishable state has been reached.



\subsection{\index{normalizing flow} Normalizing Flows}\label{ssec:NORM}

The \index{transport}transport approach from Subsection \ref{ssec:transport2} requires
invertibility of the map $g$, and efficient computation of the determinant
of the Jacobian. Invertibility of map $g$ is also useful in other
contexts. \index{normalizing flow}Normalizing flows address this issue; \emph{normalizing}
reflects the fact that distribution $ \pi' \nc $ is often a \index{Gaussian}Gaussian, whilst 
\emph{flow} connotes the breaking up of map $g$  into a sequence of
simpler maps which are themselves parameterized, rather than
parameterizing $g$ itself. 

To this end we introduce the iteration
\begin{subequations}
\begin{align}
v_{j+1}&=H(v_j;\theta_g),\\
v_0&=z,
\end{align}
\end{subequations}
and let $J \in \mathbb{N}$ be defined so that $v_J=u.$ Define 
$u=g(z)$ where $g=H \circ H \circ \dots \circ H$, the $J-$fold
composition of $H$. We assume that $H(\cdot;\theta_g)$ 
is invertible, with inverse
$H^{-1}(\cdot;\theta_g)$, and differentiable, with 
derivative $DH(\cdot;\theta_g)$. 
Assume that $z \sim \pi'$ and let $p_j(v_j)$ 
denote the density of $v_j$. Then the goal of normalizing
flow is to choose parameter $\theta_g$ in $H$ so that
$p_J \approx \pi$ and hence (approximately)
$u \sim \pi;$ this is potentially a more 
straightforward task than working with a directly parameterized $g,$ 
the approach described in Subsection \ref{ssec:transport2}.



Formula \eqref{eq:cov} shows that, since $v_j=H^{-1}(v_{j+1};\theta_g)$,
\begin{equation*}
\log p_{j+1}(v_{j+1}) = \log p_j(v_j) - {\rm det} DH(v_j;\theta_g).
\end{equation*} 
Summing over $j$ we obtain
\begin{equation*}
\log p_{J}(v_{J}) = \log p_0(v_0) - \sum_{j=0}^{J-1} {\rm det} DH(v_j;\theta_g),
\end{equation*}
and hence
\begin{equation}
\label{eq:cov2}
\log g^\sharp \pi'(u)   = \log \pi'(z) - \sum_{j=0}^{J-1} {\rm det} DH(v_j;\theta_g),
\end{equation}
where $u=g(z)$ and $v_j=g^{(j)}(z)$, the $j-$fold composition of $g$.
Note that hence $v_j=(g^{-1})^{(J-j)}(u)$, the $(J-j)-$fold 
composition of $g^{-1}.$
In particular $z$ is found as the $J-$fold
composition of $g^{-1}.$

With these relationships defined between $(z,\{v_j\})$ and $u$, and
noting that they are parameterized by $\theta_g$, we 
generalize \eqref{eq:OT99} to set 
\begin{equation}
\label{eq:OT999}
F(\theta_g)= -\bbE^{u \sim \pi} \Bigl[\log \pi'(z)- \sum_{j=0}^{J-1}
\log {\rm det}  DH(v_j;\theta_g) \Bigr].
\end{equation}
As before we set
$$\thetas_g={\rm argmin}_{\theta_g \in \Theta_g} F(\theta_g)$$
and define the resulting approximate pushforward\index{pushforward} map by 
$\gs=g(\cdot;\thetas_g).$
Note that $g(\cdot;\thetas_g)$ is found from the $J-$fold
composition of $H(\cdot;\thetas_g)$.


%\begin{remark}
%Differentiating $F(\cdot)$, a task that is complicated by the dependence
%of (for fixed $u$), $H$, $z$ and the $\{v_j\}$ on $\theta_g.$ \ds Is there something missing here? \nc
%\end{remark}



The continuum limit of \index{normalizing flow}normalizing flows
leads to differential equations
which map an initial probability distribution $\pi'$
into probability distribution $g^\sharp \pi'$ at time $t=1.$ 
To this end we define  
\begin{subequations}
\label{eq:nfode}
\begin{align}
\frac{dv}{dt}&=h(v;\theta_g),\\
v(0)&=z.
\end{align}
\end{subequations}
Noting that $v(t)$ depends on $z$ we define $g_t(z;\theta_g)=v(t)$
and $g(z;\theta_g)=g_1(z;\theta_g)=v(1).$
An advantage of the continuum perspective is that the inverse 
of map $g$ is readily computed as follows. Define the equation
\begin{subequations}
\label{eq:nfode}
\begin{align}
\frac{dw}{dt}&=-h(w;\theta_g),\\
w(0)&=u.
\end{align}
\end{subequations}
Then $g^{-1}_t(u;\theta_g)=w(t)$ and, in particular, $g^{-1}(u;\theta_g)=w(1).$




\begin{lemma}
Assume that, in \eqref{eq:nfode}, the initial condition satisfies
$z \sim \pi'$. Then 
\begin{equation}
\label{eq:cov3}
\log g^\sharp \pi'(u)   = \log \pi'(z) - \int_0^1 
\nabla \cdot h\bigl(v(s);\theta_g\bigr)ds.
\end{equation}
\end{lemma}

\begin{proof}
This may be derived from the discrete \index{normalizing flow}normalizing flow, by setting
$H(\cdot;\theta_g)=Id+\Delta t h(\cdot;\theta_g)$ where $J\Delta t=1$.
Note that this corresponds to an Euler approximation of the continuum 
picture in which $v_j \approx v(j\Delta t).$ Furthermore
$${\rm det} DH={\rm det}(I_d+\Delta t Dh)=1+\Delta t {\rm Tr} Dh
+{\mathcal O}(\Delta t^2).$$
Note that ${\rm Tr} Dh=\nabla \cdot h.$ Thus,
substituting this expression for ${\rm det} DH$
into \eqref{eq:cov2}, expanding the logarithm in powers
of $\Delta t$, summing over $j$ and letting $\Delta t \to 0$ yields
the desired result.
\end{proof}


The continuum analog of \eqref{eq:OT999} is then 
$$F(\theta_g)=
 -\bbE^{u \sim \pi} \Bigl[\log \pi'(z)- \int_0^1 
\nabla \cdot h\bigl(v(s);\theta_g\big) \, ds \Bigr],$$
where $z=g^{-1}(u;\theta_g)$ and $v(t)=g^{-1}_{1-t}(u;\theta_g).$ 
As before, up to an additive constant,
$F(\theta_g)=\dkl(\pi\|g^\sharp \pi').$
Minimizing $F$ over $\theta_g$, to obtain $\thetas_g$,
thus leads to $\gs(\cdot)=g(\cdot;\theta_g)$ and
$(\gs)^\sharp \pi' \approx \pi.$ 





\section{\index{forward!model} Learning the Forward Map}\label{sec:LForward}

Recall the \index{inverse problem}inverse problem \eqref{eq:jc0} of finding
$u$ from $y$ where
$$y=G(u)+\eta.$$
If the \index{Bayesian}Bayesian approach is adopted, and \index{MCMC}MCMC is used to generate
samples from the \index{posterior}posterior, many evaluations of $G$ may be
required to evaluate the \index{likelihood}likelihood. When $G$ is computationally 
expensive to evaluate, this may be prohibitive. 
The methods described in Section \ref{sec:FA} 
can be used to approximate the 
(scalar-valued) \index{likelihood}likelihood $\like$  resulting from $G$, 
by an approximation $ \like_{\delta}$
with small error $\delta,$ uniformly over $D  \subset \R^d $. 
Furthermore, the methods from  Section \ref{sec:FA} can all
be generalized to approximate (vector-valued) $G$
by a uniform  approximation over $D  \subset \R^d $, $G_\delta$, which
in turn results in a uniform approximation $\like_{\delta}$  of the \index{likelihood}likelihood. 
If carefully designed, then
the \index{machine learning}machine learning approximation of the \index{likelihood}likelihood will be much
faster to evaluate than the true \index{likelihood}likelihood and, because of the
approximation properties, will result in accurate \index{posterior}posterior inference,
with errors of size $\delta.$ 
Such results rely on error bounds of the form \eqref{eq:eb} which
(with high probability) can be obtained with a number $N$ of evaluations
of the \index{forward!model}forward model which is orders of magnitude smaller
than the number of evaluations required within \index{MCMC}MCMC.
The resulting method can thus be very efficient.


We now establish that the resulting approximate \index{posterior}posterior is 
indeed close to the truth, using error bounds of the form
\eqref{eq:eb} within a modification of the 
\index{well-posed}well-posedness theory from Chapter \ref{ch1}.


We denote by 
\[\like(u)=\noise\bigl(y-G(u)\bigr)\quad \text{and}\quad \like_\delta(u)=\noise\bigl(y-G_\delta(u)\bigr)\]
the true and approximate \index{likelihood}likelihoods. Thus we may define
the true and approximate \index{posterior}posterior distributions by 
\[\post^y(u)=\frac{1}{Z}\like(u)\pr(u)\quad \text{and}\quad \post_\delta^y(u)=\frac{1}{Z_\delta}\like_\delta(u)\pr(u);\]
here $Z, Z_\delta>0$ are the corresponding normalizing constants. To
prove our result about the closeness between the true \index{posterior}posterior and
the machine-learned \index{posterior}posterior we specify our assumptions.

\begin{assumption}\label{a:dh1L}
The \index{prior}prior distribution is supported on bounded open set $D \subset \Ru$.
There exist $\delta^+>0$ and $K_1,K_2<\infty$ such that, for all $\delta\in (0,\delta^+),$ 
	\begin{itemize}
	\item[(i)] $\sup_{u\in\Ru}|\sqrt{\like(u)} - \sqrt{\like_\delta(u)}|\leq K_1\delta;$
	\item[(ii)] $\sup_{u\in\Ru}(|\sqrt{\like(u)}|+|\sqrt{\like_\delta(u)}|) \le K_2.$
	\end{itemize}
\end{assumption}

This assumption follows from \eqref{eq:eb} if it is assumed that
$\like$ is uniformly bounded on $D$. Furthermore results of the
form \eqref{eq:eb} typically require continuity of $\like$ on $D$. 
Using the assumption we may state the approximation result 
for the machine-learned \index{posterior}posterior.
When combined with Lemma \ref{Lemma: hellinger}, the following theorem
guarantees that expectations computed with respect to the machine-learned
\index{posterior}posterior commit an error or order $\delta$, the magnitude of the error
in the approximate \index{likelihood}likelihood.



\begin{theorem}[\index{well-posed}Effect of Machine-Learned \index{likelihood}Likelihood on \index{posterior}Posterior] Under Assumption \ref{a:dh1L} we have
      \[\dhell(\post^y,\post_\delta^y)\leq c \delta,\quad \delta\in(0,\Delta),\]
      for some $\Delta>0$ and some $c\in(0,+\infty)$ independent of $\delta$.
      \label{thm1L}\\
\end{theorem}
%


As in the proof of the \index{well-posed}well-posedness Theorem \ref{thm1}, we first show 
a lemma which characterizes the normalization constants and their
approximation in the small $\delta$ limit.
   
     \begin{lemma}\label{lem1L} Under Assumption \ref{a:dh1L} there exist $\Delta>0$, $c_1,c_2\in(0,+\infty)$ such that 
      \[|Z-Z_\delta|\leq c_1\delta\quad \text{and}\quad Z,Z_\delta>c_2,\quad \text{for}\ \delta\in(0,\Delta).\]
      \end{lemma}
      \begin{proof} 
Since $Z=\int \like(u)\pr(u) \, du$ and
$Z_\delta=\int \like_\delta(u)\pr(u) \, du,$ 
we have
      \begin{align*}
      |Z-Z_\delta|=& \biggl| \int \bigl(\like(u)-\like_\delta(u)\bigr)\pr(u) \, du    \biggr|   \\
      \leq&\ \Big(\int \Bigl|\sqrt{\like(u)}- \sqrt{\like_\delta(u)}\Bigr|^2\pr(u) \, du\Big)^{1/2}\Big(\int \Bigl|\sqrt{\like(u)}+\sqrt{\like_\delta(u)}\Bigr|^2\pr(u) \, du\Big)^{1/2}\\
      \leq&\ \Big(\int K_1^2 \delta^2 \pr(u) \, du\Big)^{1/2}\Big(\int K_2^2\pr(u) \, du\Big)^{1/2}\\
      \leq&\ K_1 K_2\delta,\quad \delta\in(0,\delta^+). 
      \end{align*}
      Therefore, for $\delta\leq \Delta\coloneqq\min\{\frac{Z}{2K_1 K_2},\delta^+\}$, we have
      \[Z_\delta\geq Z-|Z-Z_\delta|\geq \frac{1}{2}Z.\]
      The lemma follows by taking $c_1=K_1 K_2$ and $c_2=\frac{1}{2}Z$.\\
      \end{proof}   
 
      \begin{proof}[Proof of Theorem \ref{thm1L}]
Following proof of the \index{well-posed}well-posedness Theorem \ref{thm1}, we
   decompose the total error into two contributions, reflecting respectively
the difference between $Z$ and $Z_\delta$, and the difference between 
the \index{likelihood}likelihoods $\like$ and $\like_\delta$:
      \begin{align*}
      \dhell(\post^y,\post_\delta^y)
      \leq&\ \frac{1}{\sqrt{2}}\Big\|\sqrt{\frac{\like\pr}{Z}}-\sqrt{\frac{\like\pr}{Z_\delta}}\Big\|_{L^2}+\frac{1}{\sqrt{2}}\Big\|\sqrt\frac{\like\pr}{Z_\delta}-\sqrt{\frac{\like_\delta\pr}{Z_\delta}}\Big\|_{L^2}.
      \end{align*}
      Using Lemma \ref{lem1L} we have, for $\delta\in(0,\Delta)$, 
      \begin{align*}
      \Big\|\sqrt{\frac{\like\pr}{Z}}-\sqrt{\frac{\like\pr}{Z_\delta}}\Big\|_{L^2}=&\ \Big|\frac{1}{\sqrt{Z}}-\frac{1}{\sqrt{Z_\delta}}\Big|\Big(\int \like(u)\pr(u) \, du\Big)^{1/2}\\
      =&\ \frac{|Z-Z_\delta|}{(\sqrt{Z}+\sqrt{Z_\delta})\sqrt{Z_\delta}}\\
      \leq&\ \frac{c_1}{2c_2}\delta,
      \end{align*}
      and 
      \[\Big\|\sqrt{\frac{\like\pr}{Z_\delta}} - \sqrt{\frac{\like_\delta\pr}{Z_\delta}}\Big\|_{L^2}=\frac{1}{\sqrt{Z_\delta}}\Big(\int\Bigl|\sqrt{\like(u)}- \sqrt{\like_\delta(u)}\Bigr|^2\pr(u) \, du\Big)^{1/2} \leq \sqrt{\frac{K_1^2}{c_2}}\delta.\]
      Therefore
      \[\dhell(\post^y,\post_\delta^y)\leq \frac{1}{\sqrt{2}}\frac{c_1}{2c_2}\delta+\frac{1}{\sqrt{2}}\sqrt{\frac{K_1^2}{c_2}}\delta=c \delta,\]
      with $c=\frac{1}{\sqrt{2}}\frac{c_1}{2c_2}+\frac{1}{\sqrt{2}}\sqrt{\frac{K_1^2}{c_2}}$ independent of $\delta$.
      \end{proof}








\section{Learning the \index{prior}Prior}\label{sec:LP}
Recall the \index{inverse problem}inverse problem of finding $u \in \R^d$ from $y \in \R^k$ 
when related by \eqref{eq:jc0}: $y=G(u)+\eta.$
Under the assumptions of Theorem \ref{t:bayes},
this leads to the \index{posterior}posterior distribution given by \eqref{eq:bayesformula}:
\begin{equation*}
 \post(u) = \frac{1}{Z} \noise\bigl(y - G(u)\bigr)\pr(u);
\end{equation*}
we have dropped the explicit dependence of the \index{posterior}posterior on $y$ 
for notational convenience. Now consider a setting in which the 
\index{prior}prior $\pr(u)$ is not known explicitly
and only given through samples. Assume further that $\pr=(\gd)^\sharp \pr',$
where $\gd:\R^{ \dz } \to \R^d$ and $\pr'$ is a probability density on $\R^{ \dz }.$
We have the following useful result:

\begin{lemma}
Let $ \dz  =d$ and assume that  $\gd$  is invertible. Define
\begin{equation*}
 \post'(z) = \frac{1}{Z} \noise\Bigl(y - G\bigl(\gd(z)\bigr)\Bigr)\pr'(z).
\end{equation*}
It follows that $\post=(\gd)^\sharp \post'.$ 
\end{lemma}

\begin{proof}
From Lemma \ref{lem:cov}, with $u=\gd(z)$,
\begin{align*}
(\gd)^\sharp \pi'(u)&= \bigl(\pi' \circ (\gd)^{-1}\bigr)(u) {\rm det} 
D\bigl((\gd)^{-1}\bigr)(u)\\
&= \frac{1}{Z} \noise\bigl(y - G(u)\bigr) \bigl(\rho' \circ (\gd)^{-1}\bigr)(u) 
{\rm det} D\bigl((\gd)^{-1}\bigr)(u)\\ 
&= \frac{1}{Z} \noise\bigl(y - G(u)\bigr) (\gd)^\sharp \rho'(u)\\ 
&= \frac{1}{Z} \noise\bigl(y - G(u)\bigr) \rho(u),\\
&= \pi(u) 
\end{align*}
as required.
\end{proof}

A similar result may be established even if $\dz <d$. Hence,
if pair $(\gd,\rho')$ are known, then the original \index{Bayesian!inverse problem}Bayesian 
inverse problem for $\pi$ on $\R^d$
may be converted to one for $\pi'$ on $\R^{\dz}$;
pushforward\index{pushforward} of $\pi'$ under $\gd$ yields solution to the original problem.
For this reason we concentrate on this \index{inverse problem}inverse problem in $z$-space
and the effect of having learned $\gd$ from data, and hence know it
only approximately.

In practice we typically specify $\rho'$ to be a simple measure
such as a unit \index{Gaussian}Gaussian. By means of \index{unsupervised learning}unsupervised learning
methods, such as those outlined in Subsection \ref{sec:MT},
we have access to an approximation $\gs$ to $\gd$. 
An assumption such as the following can be reasonably expected
to hold for many of these methods, if sufficient data is employed,
with high probability.
However little analysis of this kind is currently available.
We will proceed on the basis that the assumption holds.



\begin{assumption}
\label{a:g}
Assume that probability density $\rho'$ is supported on compact
set $D  \subset  \R^{\dz}.$ Then, for any $\delta>0$, there is
$\thetas_g \in \Theta_g$ such that
\begin{equation}
\label{eq:eb2}
\sup_{z \in D} |\gd(z)-\gs(z)| < \delta.
\end{equation}
\end{assumption}

In what follows, we denote by $g_{\delta}$ any function $\gs$
for which upper error bound \eqref{eq:eb2} holds.
We define 
\[\like(z)=\noise\Bigl(y-G\bigl(\gd(z)\bigr)\Bigr)\quad \text{and}\quad \like_\delta(z)=\noise\Bigl(y-G\bigl(g_{\delta}(z)\bigr)\Bigr),\]
the true and approximate \index{likelihood}likelihoods in the $z-$space
formulation of the \index{inverse problem}inverse problem. In $z-$space we also define
the true and approximate \index{posterior}posterior distributions defined by
\[\post'(z)=\frac{1}{Z}\like(z)\pr'(z)\quad \text{and}\quad \post_{\delta}'(z)=\frac{1}{Z_\delta}\like_\delta(z)\pr'(z),\]
where $Z, Z_\delta>0$ are the corresponding normalizing constants. 


\begin{theorem}[\index{well-posed}Effect of Machine-Learned 
\index{prior}Prior on \index{posterior}Posterior] 
Let Assumption \ref{a:g} hold and assume that $\nu, G$ are $C^1$ functions,
uniformly on compact sets, and that $g$ is bounded on $D$. Then we have
      \[\dhell(\post',\post_\delta')\leq c \delta,\quad \delta\in(0,\Delta),\]
      for some $\Delta>0$ and some $c\in(0,+\infty)$ independent of $\delta$.
      \label{thm1P}\\
\end{theorem}

\begin{proof}
The proof is identical to the proof of Theorem \ref{thm1L} after noting
that Assumption \ref{a:g}, together with the boundedness of $g$ and the
$C^1$ properties of $\nu, G$, imply Assumption \ref{a:dh1L}, in $z-$space.
\end{proof}




\section{Learning the \index{prior}Prior to \index{posterior}Posterior Map}\label{sec:LPrtoPo}

Consider \index{Bayes theorem}Bayes theorem written as map relating \index{prior}prior $\pr$
to \index{posterior}posterior $\post$ via the relation
\begin{align*}
 \post(u) &= \frac{1}{Z} \like(u) \pr(u),\\
Z &= \bbE^{u \sim \pr}\, \bigl[ \like(u) \bigr].
\end{align*}
This is a nonlinear map on the space of measures. We now ask
whether we can realize this nonlinear map via an invertible
transport $T$ on the \index{state-space}state-space $\R^d$ with the
property $\post=T^\sharp \pr.$ Specifically, in the notation
of Subsection \ref{ssec:transport2}, we seek to find
$\theta_g \in \Theta_g$ to minimize
$$F(\theta_g)=\dkl\bigl(\pr \| T^{-1}(\cdot; \theta_g)^\sharp \post\bigr).$$
From \eqref{eq:OT}, with $g=T^{-1}$, 
we deduce that
\begin{equation*}
F(\theta_g) 
 =  -\bbE^{u \sim \pr} \Bigl[\log \post \circ T(u;\theta_g)+ \log {\rm det}  
D_u T(u;\theta_g) \Bigr]+{\rm const},
\end{equation*}
Using the expression for the \index{posterior}posterior in terms of the \index{prior}prior, and noting
that $Z$ is constant, we may write 
\begin{equation}
\label{eq:OT50}
F(\theta_g)
 =  -\bbE^{u \sim \pr} \Bigl[\log \pr \circ T(u;\theta_g)+ 
\log \like \circ T(u;\theta_g)+\log {\rm det}  
D_u T(u;\theta_g) \Bigr]+{\rm const}.
\end{equation}
As usual we identify $\thetas_g$ with the argmin of $F$ and then
employ \index{transport}transport map $T^\star=T(\cdot;\thetas_g).$ For simplicity
we have sought the \index{posterior}posterior as transport from the \index{prior}prior. This
is natural because \index{prior}prior measures are often straightforward to sample,
and hence $F(\theta_g)$ can be evaluated by Monte Carlo, for example.
However it may be computationally expedient to seek $\post$ 
which is the pushforward\index{pushforward} 
of a different, easy-to-sample, reference measure.




\section{Discussion and Bibliography}\label{sec:IPMLBib}


The subject of \index{neural network}neural network function \index{approximation}approximation, the
core task of \index{supervised learning}supervised learning,
is overviewed in \cite{devore2021neural}.
Universal \index{approximation}approximation theorems may be found in
\cite{cybenko1989approximation,pinkus1999approximation}.
The use of \index{random features}random features was popularized as a methodology,
and analyzed rigorously, in the collection of papers
\cite{rahimi2007random,rahimi2008weighted,rahimi2008uniform}.
\index{Gaussian!process}Gaussian processes are described in \cite{williams2006gaussian}
and kernel-based methods more generally are described in
\cite{owhadi2019operator}. Error estimates for interpolation
using \index{Gaussian!process}Gaussian processes are developed in \cite{wendland2004scattered}.
The link between regression and \index{Bayesian!inversion}Bayesian inversion with
\index{Gaussian!process}Gaussian process \index{prior}priors is developed in depth in
\cite{craven1978smoothing,wahba1990spline}. A definition of
\index{MAP estimator}MAP estimator in infinite dimensions, appropriate for the
discussion in Remark \ref{rem:gpbayes}  may be found in \cite{dashti2013map}. 
We have articulated a specific link between \index{neural network}neural networks
and \index{random features}random features; a related concept underpins the subject of the
{\em neural tangent kernel} \cite{jacot2018neural}.


The subject of \index{optimal transport}optimal transport is overviewed
and systematically
developed in \cite{villani2009optimal}; computational
methodology is overviewed and developed in
\cite{peyre2017computational}.
The idea of conducting \index{unsupervised learning}unsupervised learning with 
\index{generative adversarial network}(generative adversarial networks) GANs was introduced
in \cite{goodfellow2014generative}. \index{autoencoder}Autoencoders
have a long history; see 
\cite{goodfellow2016deep,hinton1993autoencoders,schmidhuber2015deep} 
and the citations therein. Triangular transport maps
are overviewed as a method for \index{sampling}sampling in 
\cite{marzouk2016sampling}.


The idea of learning regularizers from data, to define \index{objective}objective functions
for the optimization approach to inversion, is overviewed in
\cite{arridge2019solving}. The paper \cite{soh2019learning} provides
a framework for the subject which employs structured factorizations of 
data matrices to learn semidefinite regularizers.
The paper \cite{lunz2018adversarial} develops an adversarial approach
to the problem.

The idea of learning \index{prior}prior probabilistic models from data is
described in \cite{patel2021gan} where \index{generative adversarial network}generative adversarial
networks  are used to determine a mapping from a \index{Gaussian}Gaussian
to the space of \index{prior}prior data samples. Many methods of this type
reduce the dimension of the unknown parameter space, determining
a \index{latent}latent space of low effective dimension. A different approach to learning
this mapping is to use invertible maps
\cite{kingma2018glow} and the work on
\index{normalizing flow}normalizing flows \cite{tabak2010density,song2020score};
see \cite{asim2020invertible} for application of invertible
maps to \index{prior}prior construction for inversion. 
This idea can be combined with \index{variational!Bayes method}variational inference to solve
\index{sampling}sampling problems in general, and \index{inverse problem}inverse problems in particular
\cite{rezende2015variational,sun2020deep,gabrie2021efficient,ongie2020deep}.
The use of triangular \index{transport}transport maps for \index{Bayesian!inference}Bayesian inference was introduced in \cite{el2012bayesian}.



Using emulators to speed-up forward model evaluations, for
example in the context of \index{likelihood}likelihood evaluation in \index{Bayesian!inversion}Bayesian inversion, was first introduced as a systematic methodology in \cite{sacks1989design},
and taken further in the realm of \index{Bayesian}Bayesian \index{model error}model error estimation
in \cite{kennedy2001bayesian}. The paper \cite{stuart2018posterior}
studies the use of \index{Gaussian!process}Gaussian processes for emulation, and derives
errors bounds quantifying the effect of emulation error 
on the \index{posterior}posterior; the methodology is developed for a range of applications 
in the geosciences in \cite{cleary2021calibrate}.
A specific application of the idea in climate science may 
be found in \cite{dunbar2021calibration}. Data-driven discretizations of \index{forward!model}forward models for \index{Bayesian!inversion}Bayesian inversion are studied in \cite{bigoni2020data}.

The topic of \index{clustering}clustering is overviewed in \cite{von2007tutorial}.
The paper \cite{ng2001spectral} describes an underlying mathematical
framework, based on eigenvalue perturbation theory. Understanding
large data limits of spectral clustering methods is a subject
developed in \cite{von2008consistency,hoffmann2022spectral}. 
The use of graph Laplacians, which underpin spectral \index{clustering}clustering,
in the solution of \index{inverse problem}inverse problems, is undertaken in
\cite{garcia2018continuum,dunlop2020large,trillos2017consistency,harlim2019kernel,sanz2020spde,harlim2022graph}.
The use of various machine-learning inspired \index{approximation}approximation
methods in the solution of PDEs may be found in
\cite{raissi2019physics,chen2021solving,nelsen2021random,kovachki2021neural}.




==> lectures/Lecture15.tex <==
\chapter{\Large{\sffamily{Blending \index{data assimilation}Data Assimilation and \index{machine learning}Machine Learning}}}
\label{ch:DAML}
In Part II of these notes we considered the data assimilation problem of estimating a time-evolving \index{state}state
in the setting where the dynamics governing the state-observation system
is known. It is natural to ask how to extend this to settings where
the dynamical model is itself unknown. 
This final chapter is devoted to the problem of estimating a time-evolving \index{state}state and the \index{dynamics}dynamics governing its evolution from a window of partial and noisy \index{observation}observations of the \index{state}state. Estimating jointly the \index{state}state and mathematical model governing  the \index{dynamics}dynamics  is important in \index{data assimilation}data assimilation applications where available stochastic dynamics models are inaccurate or expensive to evaluate. The accuracy of \index{data assimilation}data assimilation can be improved, for instance, by estimating parameters in the model dynamics or by learning a \index{neural network}neural network model correction; the efficiency of \index{data assimilation}data assimilation can be improved by leveraging machine-learned surrogate models that are cheap to evaluate. 

This chapter describes two algorithmic frameworks to blend \index{data assimilation}data assimilation techniques for estimating the \index{state}state with \index{machine learning}machine learning techniques for recovering model parameters or training surrogate models. 
After introducing the problem setting in Section \ref{sec:141},  Section \ref{sec:142} describes the expectation-maximization framework and an algorithmic implementation based on \index{Monte Carlo}Monte Carlo integration and \index{gradient descent}gradient descent.  Section \ref{sec:143} considers \index{Kalman filter!auto-differentiable}auto-differentiable Kalman filters, which enable blending Kalman \index{filtering}filtering algorithms with \index{gradient descent}gradient descent and \index{auto-differentiation}auto-differentiation methods. Section \ref{sec:144} closes with extensions and bibliographical remarks. The material in this chapter brings together many topics covered in these notes, including \index{optimization}optimization (Chapter \ref{chap:optimization}), \index{variational!formulation of Bayes theorem}variational formulations of \index{Bayes theorem}Bayes theorem (Chapter \ref{ch4}), \index{Monte Carlo}Monte Carlo methods (Chapters \ref{lecture5} and \ref{ch:6}), Kalman \index{filtering}filtering algorithms (Chapters \ref{chapter:DAlineargaussian} and \ref{lecture10}), and parameterizations of functions for \index{machine learning}machine learning (Chapter \ref{ch:IPML}).


\section{The Setting}\label{sec:141}
Consider \index{stochastic dynamics model}stochastic dynamics and \index{data model}data models given by 
\begin{align}
        v_{j+1} &= \Psi_\vartheta(v_j) + \xi_j, && \xi_j \sim \Nc(0, \Sigma_\beta) \index{i.i.d.} \text{ i.i.d.}, \label{eq:SSM1}\\
        y_{j+1} &= Hv_{j+1} + \eta_{j+1}, && \eta_j \sim \Nc(0, \Gamma) \index{i.i.d.}\text{ i.i.d.}, \label{eq:SSM2}
\end{align}
with \(v_0 \sim \Nc(m_0, C_0)\) independent of the independent \index{i.i.d.}i.i.d.
sequences \(\{\xi_j\}\) and  \(\{\eta_j\}\). We assume that $v_j \in \R^\Du$ and $
y_j \in \R^\Dy.$ The \index{observation}observation matrix $H$ and noise covariance $\Gamma$ in \eqref{eq:SSM2} are assumed to be known.
 The \index{stochastic dynamics model}stochastic dynamics in \eqref{eq:SSM1} are defined in terms of a deterministic map $\Psi_\vartheta$ and \index{Gaussian}Gaussian additive noise with covariance $\Sigma_\beta,$ where $\theta := \{\vartheta,\beta \}$ are model parameters. We denote  
the \index{Markov kernel}Markov kernel for the \index{dynamics}dynamics by $\Prob( \cdot \,|v_j, \theta) := \Nc \bigl(\Psi_\vartheta(v_j),\Sigma_\beta\bigr)$ and are interested in finding $\theta$ so that this \index{Markov kernel}Markov kernel approximates that of an unknown, ground-truth \index{stochastic dynamics model}stochastic dynamics model of the form
\begin{equation}\label{eq:idealizedmodel}  
   v_{j+1} = \Psi^\dagger (v_j) + \xi_j, \quad\quad  \xi_j \sim \Nc(0, \Sigma^\dagger), \quad\quad  1 \le j \le J.
\end{equation}
Once $\theta$ is found, the \index{signal}signal $\{v_j\}$ can be estimated using the \index{filtering}filtering and \index{smoothing}smoothing algorithms in Part II of these notes with \index{stochastic dynamics model}stochastic dynamics \eqref{eq:SSM1} and \index{data model}data model \eqref{eq:SSM2}.
The role of the parameter $\beta$ is to enable estimating the unknown covariance $\Sigma^\dagger.$ We consider three motivating examples for the interpretation of the parameter $\vartheta,$ of the parameterized map $\Psi_\vartheta,$ and of the relationship between the map $\Psi_\vartheta$ and the ground-truth deterministic map $\Psi^\dagger.$ 

\begin{example}[Parameterized Dynamics]
$\Psi^\dagger = \Psi_{\vartheta^\dagger}$ is parameterized, but the true parameter $\vartheta^\dagger$ is unknown and needs to be estimated. For instance, $\Psi^\dagger$ may be defined by time-discretization of a parameterized system of differential equations and we may be interested in estimating $\vartheta^\dagger$ from \index{observation}observations $\{y_j\}.$
\end{example}

\begin{example}[Fully-Unknown Dynamics]
There are settings in which $\Psi^\dagger$ is fully unknown and $\vartheta$ represents the parameters of a \index{neural network}neural network, \index{random features}random features, or \index{Gaussian!process}Gaussian process surrogate model $\Psi_\vartheta$ for $\Psi^\dagger;$ see Chapter \ref{ch:IPML} for background on these parameterizations of functions. The goal is to find an accurate surrogate model $\Psi_\vartheta$. Even if $\Psi^\dagger$ is fully known, a surrogate model, or \emph{emulator}, may be much cheaper to evaluate, enabling the use of large sample size for particle filters or ensemble Kalman methods. Similar computational considerations motivated learning the forward map for inverse problems in Chapter \ref{ch:IPML}. 
\end{example}

\begin{example}[Model Correction]
$\Psi^\dagger$ is unknown, but we have access to an inaccurate model $\Psi^{\text{approx}} \approx \Psi^\dagger$. Here $\vartheta$ represents the parameters of a \index{neural network}neural network, \index{random features}random features, or \index{Gaussian!process}Gaussian process $\Psi^{\text{correction}}_\vartheta$ used to correct the inaccurate model $\Psi^{\text{approx}}$. The goal is to learn $\vartheta$ so that $\Psi_\vartheta \triangleq \Psi^{\text{approx}} + \Psi^{\text{correction}}_\vartheta$ approximates $\Psi^\dagger$ accurately. Learning model corrections is important in applications where available models have moderate predictive accuracy.  
For instance, fine scales of the \index{state}state may not be resolved accurately due to computational constraints and we may be interested in learning from data a surrogate model which accounts for the unresolved scales of the system.  
\end{example}


For a given and fixed integer $J,$ we define, following the notation in Chapter \ref{lecture7},
\begin{equation*}
\V := \{v_0, \ldots, v_J\}, \quad \quad  \Y := \{y_1, \ldots, y_J\}.
\end{equation*}
Note that $\V \in \R^{\Du(J+1)}$ and $\Y \in \R^{\Dy J}$. 
In contrast to the \index{supervised learning}supervised learning setting in Chapter \ref{ch:IPML}, here we do not assume to have direct data $\{ v^{(n)}, \Psi^\dagger(v^{(n)})\}_{n=1}^N$ to learn the map $\Psi^\dagger.$ Instead, we assume to have only access to data $Y$ obtained from indirect and noisy measurement of a trajectory $V$ from the signal. 
However, this new learning task can also be cast as an optimization problem, and to that end we adopt a \index{maximum likelihood estimation}\emph{maximum likelihood estimation} approach to estimate $\theta.$ That is, we seek to find $\theta$ that maximizes the \index{likelihood}likelihood function of $\theta$ given the observed data $Y:$
\begin{equation}
\Prob(Y | \theta) = \int \Prob (V, Y |\theta) \, dV = \int \Prob (Y | V) \Prob (V | \theta) \, dV.
\end{equation}
In the last equation we used that $\Prob (Y | V, \theta) = \Prob (Y | V);$ here and throughout this chapter integrals are over $\R^{\Du(J+1)}$ unless otherwise noted. Evaluating the \index{likelihood}likelihood function $\Prob(Y | \theta)$ is challenging due to the unobserved, or  \index{latent}\emph{latent}, variable $V$. Therefore, in practice we may seek to maximize a lower bound or an approximation  
of the \index{likelihood}likelihood function. 
 
 
Whilst evaluating the likelihood is often challenging, we will use in the sequel that the joint distribution of $V$ and $Y$ admits the characterization
\begin{align}\label{eq:joint}
\begin{split}
\log  \Prob(V,Y | \theta)  &= \log\Prob (Y|V)  + \log \Prob (V|\theta) \\
& =  -  \frac{1}{2} \displaystyle{\sum_{j=0}^{J-1}}|y_{j+1} - Hv_{j+1}|_{\Gamma}^2 -\frac12 \text{det} \log(\Sigma_\beta)\\
 &-  \frac{1}{2}|v_0-m_0|^2_{C_0} - \frac{1}{2}  \sum_{j=0}^{J-1} |v_{j+1} - \Psi_\vartheta(v_j)|^2_{\Sigma_\beta}  + c,
\end{split}
\end{align}
where $c$ is a constant independent of $V,$ $Y$ and $\theta.$
The next two sections consider two algorithmic frameworks to approximately compute the \index{maximum likelihood estimation}maximum likelihood estimator.




\section{The \index{expectation-maximization}Expectation-Maximization Framework}\label{sec:142}
 The \index{expectation-maximization}expectation-maximization (\index{EM}EM) algorithm is a general-purpose approach to \index{maximum likelihood estimation}maximum likelihood estimation with \index{latent}latent variables.  We derive it here in general terms and then specify it to the problem of joint estimation of \index{state}state and \index{dynamics}dynamics model parameters $\theta$.  Central to the abstract derivation of the \index{EM}EM algorithm is the following lower bound of the \index{likelihood}log-likelihood function, obtained using \index{Jensen inequality}Jensen inequality:
\begin{align*}
\log \Prob (Y | \theta) &= \log \int \Prob (V, Y| \theta) \, dV \\ 
&  = \log \int \frac{\Prob (V, Y| \theta)}{q(V)} q(V) \, dV \\ 
& \ge \int\log\biggl( \frac{\Prob (V, Y| \theta)}{q(V)} \biggr)  q(V)  \, dV = :\mathcal{L}(q, \theta),
\end{align*}
where $q$ is any pdf over the \index{latent}latent variables $V$ with compatible support. 
In fact, the following theorem shows that the difference between $\log \Prob (Y | \theta)$ and $\mathcal{L}(q, \theta)$ is given by the \index{divergence!Kullback-Leibler}Kullback-Leibler divergence $\dkl \bigl( q \| \Prob(V|Y,\theta)\bigr),$ which is always non-negative. Notice that the proof is identical to that of the \index{variational!formulation of Bayes theorem}variational formulation of \index{Bayes theorem}Bayes theorem in Chapter \ref{ch4}.

\begin{theorem}[\index{likelihood}Likelihood Characterization for \index{EM}EM Framework]\label{th:EMlikecharacterization}
It holds that 
\begin{equation*}
\log \Prob (Y | \theta) = \mathcal{L}(q, \theta) + \dkl \bigl( q \| \Prob(V|Y,\theta)\bigr).
\end{equation*}
\end{theorem}
\begin{proof}
Using the definition of $\mathcal{L}(q, \theta),$ product rule, and the definition of the \index{divergence!Kullback-Leibler}Kullback-Leibler divergence in Chapter \ref{ch4}, we have
\begin{align*}
\mathcal{L}(q, \theta) &= \int\log\biggl( \frac{\Prob (V, Y)| \theta)}{q(V)} \biggr)  q(V)  \, dV \\
& = \int \log \biggl( \frac{\Prob(V|Y,\theta)}{q(V)} \biggr) q(V) \, dV + \int \log \Prob(Y|\theta) q(V) \, dV \\
& = - \dkl \bigl(q \| \Prob(V |Y, \theta) \bigr) + \log \Prob(Y|\theta),
\end{align*}
as desired.
\end{proof}

Theorem \ref{th:EMlikecharacterization} motivates an iterative approach to maximize the \index{likelihood}log-likelihood function $\log \Prob (Y | \theta),$ which is equivalent to maximizing the \index{likelihood}likelihood $\Prob (Y | \theta)$ since the logarithm is an increasing function.
Given  the current iterate  $\theta_\ell,$ we obtain the next iterate  $\theta_{\ell+1}$ in two steps, maximizing in turn the two components of the lower bound:
\begin{enumerate}
\item First,  we find $q_\ell(V)$ that maximizes the lower bound $\mathcal{L}(q, \theta_\ell)$  over pdf $q.$  From Theorem \ref{th:EMlikecharacterization}, 
$$\log \Prob (Y | \theta_\ell) = \mathcal{L}(q, \theta_\ell) + \dkl \bigl( q \| \Prob(V|Y,\theta_\ell)\bigr),$$
and it follows that maximizing $\mathcal{L}(q, \theta_\ell)$ or minimizing $\dkl \bigl( q \| \Prob(V|Y,\theta_\ell)\bigr)$ over $q$ are equivalent. Since the \index{divergence!Kullback-Leibler}Kullback-Leibler divergence is minimized when both arguments agree, we obtain that $q_\ell(V) = \Prob(V|Y,\theta_\ell).$
\item Second, we  obtain $\theta_{\ell + 1}$ by maximizing the lower bound  $\mathcal{L}(q_\ell, \theta)$ over $\theta.$ Note that 
\begin{equation}
\mathcal{L}(q_\ell, \theta) = \int \log\Prob(V, Y | \theta) \Prob(V|Y, \theta_\ell) \, dV + c,
\end{equation}
where $c$ is independent of $\theta.$ Hence, the quantity to maximize is the expected value of the joint log-density $\log  \Prob (V, Y | \theta)$ with respect to $q_\ell(V) = \Prob(V|Y, \theta_\ell).$
\end{enumerate}


Combining these two steps gives the \index{EM}EM framework, summarized in Algorithm \ref{alg:EM} below. Figure \ref{fig:EM} illustrates how each new iterate is obtained by maximizing a lower bound on the \index{likelihood}log-likelihood. 
\begin{figure}[h]
  \begin{center}
    \includegraphics[width=0.6\textwidth]{figures/EM2}
  \end{center}
  \caption{Iterates of the \index{EM}EM algorithm. The blue and red lines represent \index{likelihood}log-likelihood lower bounds as functions of $\theta.$ Notice that they lie below the \index{likelihood}likelihood, but $\Prob(Y| \theta_\ell) = \mathcal{L}(q_\ell, \theta_\ell)$ since by design $\dkl \bigl(q_\ell \| \Prob(V|Y, \theta_\ell) \bigr) = 0$ for all $\ell \ge 0.$ 	} \label{fig:EM}
\end{figure}
\begin{algorithm}
\caption{\label{alg:EM} Expectation Maximization}
\begin{algorithmic}[1]
%\vspace{0.1in}
\STATE {\bf Input}:  Initialization $\theta_0.$
\STATE For $\ell = 0, 1, \ldots, L-1$ do the following expectation and maximization steps:
\STATE {\bf E-Step}: Compute 
\begin{align*}
\Expect^{V \sim  \Prob(V|Y, \theta_\ell)} \Bigl[ \log \Prob(V, Y | \theta) \Bigr]= \int \log \Prob(V, Y | \theta) \Prob(V|Y, \theta_\ell) \, dV. 
\end{align*}
\vspace{-0.5cm}
\STATE{{{\bf M-Step}}}: Compute 
\begin{equation*}
\theta_{\ell+1} = \arg \max_\theta \Expect^{V \sim  \Prob(V|Y, \theta_\ell)} \Bigl[ \log \Prob(V, Y | \theta) \Bigr].
\end{equation*}
%and replace $\ell$ by $\ell+ 1.$
\STATE{\bf Output}: Parameter $\theta^L.$
\end{algorithmic}
\end{algorithm}
\FloatBarrier


The following result shows that the \index{EM}EM framework has the desirable property that the \index{likelihood}likelihood function increases monotonically along iterates $\theta_\ell.$ 

\begin{theorem}[Monotonic Increase of \index{likelihood}Likelihood along \index{EM}EM Iterates]\label{th:EMmonotone}
Let $\{\theta_\ell \}_{\ell = 0}^{L-1}$ by the iterates of the EM Algorithm \ref{alg:EM}. Then, for $0 \leq \ell \leq L-1,$ it holds that 
\begin{equation}
\log \Prob(Y | \theta_\ell) \le \log \Prob (Y | \theta_{\ell + 1}).
\end{equation}
\end{theorem}
\begin{proof}
Let $q_\ell(V) = \Prob(V|Y, \theta_\ell).$  Using the \index{likelihood}log-likelihood characterization in Theorem \ref{th:EMlikecharacterization}, it holds that 
\begin{align*}
\log \Prob (Y | \theta_{\ell + 1}) &=\mathcal{L}(q_\ell, \theta_{\ell + 1}) + \dkl \bigl( q_\ell \| \Prob(V|Y,\theta_{\ell + 1})\bigr) \\ 
&\ge \mathcal{L}(q_\ell, \theta_{\ell}) +  \dkl \bigl( q_\ell \| \Prob(V|Y,\theta_{\ell + 1})\bigr) \\
&\ge \mathcal{L}(q_\ell, \theta_{\ell})  + \dkl \bigl( q_\ell \| \Prob(V|Y,\theta_{\ell })\bigr) \\
& = \log \Prob (Y | \theta_{\ell}).
\end{align*}
The first inequality follows because $\theta_{\ell + 1} = \arg \max_\theta \mathcal{L}(q_\ell, \theta);$ the second because $\dkl \bigl(q_\ell \| \Prob(V|Y, \theta_\ell) \bigr) = 0$ since $q_\ell = \Prob(V|Y, \theta_\ell),$ while $\dkl \bigl( q_\ell \| \Prob(V|Y,\theta_{\ell+1 })\bigr) \ge 0.$ 
\end{proof}

\begin{remark}
\label{rem:em}
As a consequence of Theorem \ref{th:EMmonotone} it is possible to deduce ---under mild assumptions--- that the iterates $\theta_\ell$ of the \index{EM}EM algorithm converge, as $\ell \to \infty,$ to a local maximizer of the \index{likelihood}likelihood function. It is important to note, however, that the expectation in the E-step and the \index{optimization}optimization in the M-step are often intractable. \index{Monte Carlo}Monte Carlo, \index{filtering}filtering, or \index{smoothing}smoothing algorithms may be employed to approximate the E-step, and \index{optimization}optimization algorithms to approximate the M-step. Such approximations can cause loss of monotonicity and convergence guarantees. 
\end{remark}

Let us now return to the problem of jointly estimating \index{state}state and \index{dynamics}dynamics. To illustrate the application of the \index{EM}EM algorithm in this setting, we consider \index{Monte Carlo}Monte Carlo methods for the E-step and \index{gradient descent}gradient descent \index{optimization}optimization for the M-step. 

For the E-step, recall equation \eqref{eq:joint} to see that 
\begin{equation}\label{eq:Erisk}
\Expect^{V \sim  \Prob(V|Y, \theta_\ell)} \Bigl[ \log \Prob(V, Y | \theta) \Bigr] = -\frac12 \log \text{det}(\Sigma_\beta)  - \frac{1}{2} \int  \sum_{j=0}^{J-1} |v_{j+1} - \Psi_\vartheta(v_j)|^2_{\Sigma_\beta} \Prob(V|Y, \theta_\ell) dV + c,
\end{equation}
where $c$ is independent of $\theta.$ Thus, given (approximate) samples $\{V^{(n)}\}_{n=1}^N$ from $\Prob(V|Y, \theta_\ell),$ we may use \index{Monte Carlo}Monte Carlo integration to approximate
\begin{equation}\label{eq:Eempiricalrisk}
\Expect^{V \sim  \Prob(V|Y, \theta_\ell)} \Bigl[ \log \Prob(V, Y | \theta) \Bigr] \approx -\frac12 \log \text{det}(\Sigma_\beta)  - \frac{1}{2} \frac{1}{N} \sum_{n=1}^N \sum_{j=0}^{J-1} |v_{j+1}^{(n)} - \Psi_\vartheta(v_j^{(n)})|^2_{\Sigma_\beta}.
\end{equation}
For the $M$-step, we notice that given $\vartheta,$ the above expression can be explicitly maximized over $\beta;$ however, to optimize over $\vartheta$ we need to resort to \index{optimization}optimization methods. The following algorithm summarizes an \index{EM}EM implementation for learning \index{dynamics}dynamics and \index{state}states using \index{Monte Carlo}Monte Carlo and \index{gradient descent}gradient descent.  



\begin{algorithm}
\caption{\label{alg:EM2} \index{expectation-maximization}Expectation-Maximization with \index{Monte Carlo}Monte Carlo and \index{gradient descent}Gradient Descent}
\begin{algorithmic}[1]
\STATE {\bf Input}:  Initialization $\theta^0 = (\vartheta^0, \beta^0).$ Rule to choose \index{gradient descent}gradient descent step-sizes $\{\alpha_i\}_{i = 1}^\mathcal{I}.$
\STATE For $\ell = 0, 1, \ldots, L-1$ do the following expectation and maximization steps:
\STATE {\bf E-Step}: Obtain (approximate) samples $\{V^{(n)}\}_{n=1}^N$ from $\Prob(V|Y, \theta_\ell).$ 
\STATE{{{\bf M-Step}}}: 
\STATE Set $$\Sigma_{\beta^{\ell+1}} = \frac{1}{NJ} \sum_{n=1}^N \sum_{j=0}^{J-1} \Big( v_{j+1}^{(n)} - \Psi_{\vartheta^{\ell}}(v_{j}^{(n)}) \Big) \Big( v_j^{(n)} - \Psi_{\vartheta^{\ell}}(v_{j}^{(n)}) \Big)^{\top}$$
and define
$$\J(\vartheta, \{V^{(n)}\}_{n=1}^N) \triangleq \frac{1}{NJ} \sum_{n=1}^N  \sum_{j=0}^{J-1} |v_{j+1}^{(n)} - \Psi_\vartheta(v_j^{(n)})|^2_{\Sigma_{\beta^{\ell +1}}}.$$
\STATE Initialize $\vartheta^{\ell,0}=\vartheta^\ell.$
\STATE For $i=0,\dots,\mathcal{I}-1$ do:
\STATE $\vartheta^{\ell,i+1} = \vartheta^{\ell,i} - \alpha_i \nabla \J(\vartheta^{\ell,i}, \{ V^{(n)} \}_{n=1}^N). $ 
\STATE Set $\vartheta^{\ell+1} = \vartheta^{\ell,\mathcal{I}}$.
\STATE{\bf Output}: Approximation $\theta^L$ to the \index{maximum likelihood estimation}maximum likelihood estimator.
\end{algorithmic}
\end{algorithm}
\FloatBarrier
The \index{signal}signal $\{v_j\}$ can be estimated by performing \index{data assimilation}data assimilation with the \index{stochastic dynamics model}stochastic dynamics and \index{data model}data models  \eqref{eq:SSM1} and \eqref{eq:SSM2} with learned parameter $\vartheta^L$ and covariance model $\Sigma_{\beta^L}.$

\begin{remark}
In analogy to the supervised learning task studied in Chapter \ref{ch:IPML}, equation \eqref{eq:Erisk} may be conceptually interpreted as defining a risk for the parameter $\theta;$ here the distribution $\Prob(V|Y,\theta_\ell),$ which represents our available knowledge on the distribution of the latent variable $V$ given data $Y$ and parameter estimate $\theta^\ell,$ plays an analogous role to $\Upsilon$ in Chapter \ref{ch:IPML}. Then, \eqref{eq:Eempiricalrisk} can be interpreted as an empirical risk, defined via approximate samples $V^{(n)} \sim \Prob(V|Y, \theta_\ell).$ These samples may be obtained, for instance, using the  \index{MCMC}MCMC methods described in Chapter \ref{ch:6}. Alternately, ensemble Kalman methods may be employed, with the proviso that, as discussed in Chapter \ref{lecture10}, they can yield accurate posterior samples only in approximately \index{linear-Gaussian setting}linear-Gaussian settings. Finally, notice that the implementation of the EM framework in Algorithm \ref{alg:EM2} treats differently the parameters $\vartheta$ and $\beta$ in the M-step. This is because \index{optimization}optimization of the empirical risk over $\Sigma_\beta$ admits a closed form solution, but optimization algorithms such as gradient descent are needed to optimize $\vartheta$ for general parameterization $\Psi_\vartheta$ of the dynamics. 
\end{remark}


\section{\index{Kalman filter!auto-differentiable} Auto-Differentiable Kalman Filters}\label{sec:143}
In Chapter \ref{lecture10} we studied \index{Kalman filter!extended}extended and ensemble \index{Kalman filter!ensemble}Kalman filtering algorithms that combine a \index{Gaussian!approximation}Gaussian approximation
\begin{equation}\label{eq:Gaussianpred}
\Prob (v_{j+1}| Y_j, \theta) \approx \Nc \bigl(\widehat{m}_{j+1}(\theta),\widehat{C}_{j+1}(\theta) \bigr)
\end{equation}
for the predictive distribution with a linear-Gaussian \index{Gaussian} \index{data model}data model to derive an approximation 
\begin{equation}
\Prob (v_{j+1}| Y_{j+1}, \theta) \approx \Nc \bigl( m_{j+1}(\theta), C_{j+1}(\theta)\bigr)
\end{equation}
of the \index{filtering!distribution}filtering distribution. These \index{Gaussian!approximation}Gaussian approximations can be accurate if the noise in the \index{dynamics}dynamics and the \index{observation!noise} observations are small, or the map $\Psi_\vartheta$ is approximately linear. 
In this section we show how the \index{Gaussian!ansatz}Gaussian ansatz \eqref{eq:Gaussianpred} can be leveraged to produce a Kalman-based approximation of the \index{likelihood}log-likelihood function $\log \Prob(Y|\theta)$ and thereby an algorithm for \index{maximum likelihood estimation}maximum likelihood estimation. The derivation rests upon the following characterization of the \index{likelihood}log-likelihood function under a \index{Gaussian!ansatz}Gaussian ansatz.
\begin{theorem}[\index{likelihood}Likelihood Characterization under \index{Gaussian}Gaussian Predictive Distribution]
Suppose that, for each $0 \le j \le J-1,$ the predictive distribution $\Prob (v_{j+1}| Y_j, \theta)$ of the stochastic dynamics and data models \eqref{eq:SSM1} and \eqref{eq:SSM2} is \index{Gaussian}Gaussian with mean $\widehat{m}_{j+1}(\theta)$ and covariance $\widehat{C}_{j+1}(\theta).$ Then the \index{likelihood}log-likelihood function admits the following characterization 
\begin{equation}\label{eq:kalmanlikelihood}
\log \Prob (Y | \theta) = - \frac12 \sum_{j = 0 }^{J-1} |y_{j+1} - H\widehat{m}_{j+1}(\theta)|_{S_{j+1}(\theta)}^2 - \frac12 \sum_{j=0}^{J-1} \log \text{\emph{det}} \bigl(S_{j+1}(\theta)\bigr),
\end{equation}
where $S_{j+1}(\theta) = H \widehat{C}_{j+1}(\theta) H^\top + \Gamma.$
\end{theorem}
\begin{proof}
We have  
\begin{align*}
\log \Prob(Y|\theta) &= \sum_{j=0}^{J-1} \log  \Prob(y_{j+1}|Y_{j},\theta),
\end{align*}
where we use the convention that  $Y_0 := \emptyset$ 
so that conditioning to $Y_0$ does not provide any information. 
Now conditioning in the \index{data model}data model
$$y_{j+1}  = H v_{j+1} + \eta_{j+1},$$
we see that
\begin{align*}
\Expect[y_{j+1} |Y_j ] &= \Expect[H v_{j+1} + \eta_{j+1} |Y_j] = H \widehat{m}_{j+1}(\theta), \\
\text{Cov}[y_{j+1} | Y_j ] & = \text{Cov}[ H v_{j+1} + \eta_{j+1}|Y_j ] = H \widehat{C}_{j+1}(\theta) H^\top + \Gamma.
\end{align*}
Moreover, $\Prob(y_{j+1} |Y_j)$ is \index{Gaussian}Gaussian. The result follows. 
\end{proof}

Thus, for any value of $\theta$, we may obtain an \emph{approximation} of the log-likelihood $\log \Prob(Y | \theta)$ by running a Kalman filtering algorithm, obtaining predictive means and covariances $\widehat{m}_{j+1}(\theta),\widehat{C}_{j+1}(\theta),$ for $0 \le j \le J-1$, and using \eqref{eq:kalmanlikelihood}. Moreover, an approximation of the log-likelihood gradient at $\theta$ can be obtained auto-differentiating through our Kalman-based likelihood estimate. Automatic-differentiation involves repeated application of chain rule on elementary operations and enables computing derivatives accurately to working precision. Auto-differentiable Kalman filters use these estimates of the log-likelihood gradients to conduct gradient descent. The procedure is summarized in Algorithm \ref{alg:autodiff}.


\begin{algorithm}
\caption{\label{alg:autodiff} Auto-Differentiable Kalman Filter}
\begin{algorithmic}[1]
%\vspace{0.1in}
\STATE {\bf Input}:  Initialization $\theta^0,$ rule to choose step-sizes $\{\alpha_\ell\}_{\ell = 0}^{L-1}.$
\STATE For $\ell = 0, 1, \ldots, L-1$ do the following Kalman \index{filtering}filtering and \index{gradient descent}gradient descent steps:
\STATE {\bf Kalman Filtering}: Run a Kalman \index{filtering}filtering algorithm to obtain predictive means and covariances $\widehat{m}_{j+1}(\theta^\ell),\widehat{C}_{j+1}(\theta^\ell),$ for $0 \le j \le J-1.$ Set
$$ \J(\theta^\ell): =  \frac12 \sum_{j = 0 }^{J-1} |y_{j+1} - H\widehat{m}_{j+1}(\theta^\ell)|_{S_{j+1}(\theta^\ell)}^2 + \frac12 \sum_{j=0}^{J-1} \log \text{det} \bigl(S_{j+1}(\theta^\ell)\bigr).$$
\STATE {\bf \index{gradient descent}Gradient Descent:} \index{auto-differentiation}Auto-differentiate the map $\theta^\ell \mapsto \J(\theta^\ell)$ to obtain a gradient estimate $\nabla \J(\theta^\ell).$  Set 
	\begin{align}
	\theta^{\ell + 1} = \theta^\ell - \alpha_\ell \nabla \J(\theta^\ell).
	\end{align}
\STATE{\bf Output}: Approximation $\theta^L$ to the \index{maximum likelihood estimation}maximum likelihood estimator. 
\end{algorithmic}
\end{algorithm}
\FloatBarrier
The \index{signal}signal $\{v_j\}$ can be estimated by performing \index{data assimilation}data assimilation with \index{stochastic dynamics model}the stochastic dynamics and \index{data model}data models  \eqref{eq:SSM1} and \eqref{eq:SSM2} with learned parameter $\theta^L.$

\begin{remark}
Notice that in the EM Algorithm \ref{alg:EM2} each posterior sample $\{V^{(n)} \}_{n=1}^N$ is used to perform $\mathcal{I}$ gradient descent steps in the M-Step, with the goal of maximizing the lower bound $\mathcal{L}(q_\ell, \theta).$ In contrast, in the auto-differentiable Kalman filter Algorithm \ref{alg:autodiff}, each run of a Kalman filtering algorithm is used to produce an estimate of the log-likelihood gradient, and a gradient descent is taken. 
\end{remark}



\section{Discussion and Bibliography}\label{sec:144}

In this chapter we have introduced two computational frameworks for joint state and parameter estimation: the EM algorithm and \index{Kalman filter!auto-differentiable}auto-differentiable filters. Both frameworks find the parameters in the \index{dynamics}dynamics by approximating the \index{maximum likelihood estimation}maximum likelihood estimator, and then use a \index{filtering}filtering or \index{smoothing}smoothing algorithm to recover the \index{state}state. This final section provides bibliographical context for the algorithms considered in this chapter, and briefly discusses other computational methods that do not stem from a \index{maximum likelihood estimation}maximum likelihood formulation.

%MLE -EM
The EM framework for  \index{maximum likelihood estimation}maximum likelihood estimation was introduced in \cite{dempster1977maximum}.
Embedding of the \index{EnKF}EnKF and the \index{Kalman smoother!ensemble}ensemble Kalman smoother (EnKS) into the \index{EM}EM algorithm was proposed in \cite{tandeo2015offline,ueno2014iterative, dreano2017estimating, pulido2018stochastic}, with a focus on estimation of error covariance matrices.  The E-step is approximated with an EnKS under the \index{Monte Carlo}Monte Carlo EM framework \cite{wei1990monte}. In addition, \cite{brajard2020combining, nguyen2019like} incorporate machine learning techniques in the M-step to train \index{neural network}neural network surrogate models. The paper \cite{bocquet2020bayesian} proposes \index{Bayesian}Bayesian estimation of model error statistics, together with a \index{neural network}neural network emulator for the \index{dynamics}dynamics. On the other hand, \cite{ueno2016bayesian,cocucci2021model} consider online \index{EM}EM methods for error covariance estimation with \index{EnKF}EnKF. Although gradient information is used during the M-step to train the surrogate model \cite{brajard2020combining, nguyen2019like,bocquet2020bayesian},  these methods do not \index{auto-differentiation}auto-differentiate through the \index{EnKF}EnKF. 

%MLE-autodiff
Our presentation of auto-differentiable Kalman filters follows  \cite{chen2021auto}, which proposes and analyzes an approach for joint \index{state}state and parameter estimation that leverages gradient information of an \index{EnKF}EnKF estimate of the \index{likelihood}likelihood. 
\index{EnKF}EnKFs for derivative-free \index{maximum likelihood estimation}maximum likelihood estimation are studied in \cite{stroud2010ensemble,pulido2018stochastic}. An empirical comparison of the \index{likelihood}likelihood computed using the  \index{EnKF}EnKF and other \index{filtering}filtering algorithms is made in \cite{carrassi2017estimating}; see also \cite{hannart2016dada,metref2019estimating}. The paper \cite{drovandi2021ensemble} uses \index{EnKF}EnKF \index{likelihood}likelihood estimates to design a pseudo-marginal \index{MCMC}MCMC method  for \index{Bayesian!inference}Bayesian inference of model parameters. The works \cite{stroud2007sequential,stroud2018bayesian} propose online \index{Bayesian}Bayesian parameter estimation using the \index{likelihood}likelihood computed from the \index{EnKF}EnKF under a certain family of conjugate distributions. 


While our discussion has focused on ensemble Kalman methods, \index{particle filter}particle filters can also be employed for joint \index{state}state and parameter estimation. \index{particle filter}Particle filters give an unbiased estimate of the data \index{likelihood}likelihood \cite{del2004feynman,andrieu2010particle}. Based upon this \index{likelihood}likelihood estimate, a particle \index{MCMC}MCMC \index{Bayesian}Bayesian parameter estimation method is designed in \cite{andrieu2010particle}. Although \index{particle filter}particle filter \index{likelihood}likelihood estimates are unbiased, they suffer from two potential drawbacks that limit their applicability to some problems. First, their variance can be large, as they inherit the weight degeneracy of \index{importance sampling}importance sampling in high dimensions \cite{snyder2008obstacles,agapiou2017importance,sanz2018importance,sanz2020bayesian} ---see Chapters \ref{ch11} and \ref{ch12} for further background on this subject. Second, while the forecast and analysis steps of \index{particle filter}particle filters can be \index{auto-differentiation}auto-differentiated, the \index{resampling}resampling steps involve discrete distributions that cannot be handled by the reparameterization trick, as discussed in \cite{chen2021auto}. For this reason, previous differentiable \index{particle filter}particle filters omit \index{auto-differentiation}auto-differentiation of the \index{resampling}resampling step \cite{naesseth2018variational,maddison2017filtering,le2017auto}, introducing a bias.

%Variational Inference
An alternative to \index{maximum likelihood estimation}maximum likelihood estimation is to optimize a lower bound of the data \index{likelihood}log-likelihood with \index{variational!Bayesian method}variational inference \cite{bishop,kingma2013auto,ranganath2014black}. The \index{posterior}posterior distribution over the \index{latent}latent \index{state}states is approximated with a parametric distribution and is jointly optimized with model parameters defining the \index{dynamics}dynamics model. In this direction, \index{variational!Bayesian method}variational sequential \index{Monte Carlo}Monte Carlo methods  \cite{naesseth2018variational,maddison2017filtering,le2017auto} construct the lower bound using a \index{particle filter}particle filter. Moreover, the proposal distribution of the \index{particle filter}particle filter is parameterized and jointly optimized with model parameters. 
Although \index{variational!Bayesian method}variational sequential \index{Monte Carlo}Monte Carlo methods provide consistent data \index{likelihood}log-likelihood estimates, they suffer from the same two potential drawbacks as \index{likelihood}likelihood-based \index{particle filter}particle filter methods. A recent work \cite{ishizone2020ensemble} proposes blending \index{variational!Bayesian method}variational sequential \index{Monte Carlo}Monte Carlo and \index{EnKF}EnKF with an \index{importance sampling}importance sampling-type lower bound estimate, which is effective if the \index{state}state dimension is small. Other works that build on the \index{variational!Bayesian method}variational inference framework include \cite{krishnan2017structured,rangapuram2018deep,fraccaro2017disentangled}. An important challenge is to obtain suitable parameterizations of the \index{posterior}posterior, especially when the \index{state}state dimension is high. For this reason, a restrictive \index{Gaussian}Gaussian parameterization with a diagonal covariance matrix is often used in practice \cite{krishnan2017structured,fraccaro2017disentangled}.

%State augmentation
Another alternative approach to maximum likelihood estimation is to concatenate state and parameters into an augmented \index{state-space}state-space, and employ the data assimilation methods in Part II of these notes in the augmented state-space. This approach requires one to design a pseudo-dynamic for the parameters, which can be challenging when certain types of parameters (e.g., error covariance matrices) are involved \cite{stroud2007sequential,delsole2010state} or if the dimension of the parameters is high.
The use of \index{EnKF}EnKF for joint learning of \index{state}state and model parameters by \index{state augmentation}\emph{state augmentation} was introduced in \cite{anderson2001ensemble}.

%learning dynamics
Beyond the problem of joint parameter and state estimation, the development of data-driven \index{machine learning} frameworks for learning \index{dynamical system}dynamical systems is a very active research area. We refer to \cite{brunton2019data,gottwald2021supervised,harlim2021machine,raissi2018multistep}  for recent methods that do not rely on the \index{EM}EM algorithm, \index{auto-differentiation}auto-differentiation of \index{filtering}filtering methods, or \index{variational!Bayesian method}variational inference.




==> notes_3.8.18 <==
March 8th--16th 2018.


o First citation is in a different font from the others

o Make Remarks end with a \qed

o Make Examples end with a \qed

o Make citations numerical [34] etc.

o Make sure all Definitions have the defined object in italics and end
with a \qed.

o The \varphi in Examples 6.2 and 6.5 needs to be plain \phi to match
figure legend (or change figure to \varphi). Problem is that
\phi is appearing as \varphi in this font.

o Bibliography/bibtex not working. I added new references to 
references.bib (eg cotter2013) and its not getting incorporated.
Maybe related to:
"I found no \bibdata command---while reading file final_merged.aux
I found no \bibstyle command---while reading file final_merged.aux"
Similar for {iglesias2013ensemble}

o Do we know who latexed up Lecture 12? They added Theorem 12.1, I think, or did
I cover it? If they added it then we should be crediting that person
explicitly in the introduction?

o Figures 19 and 20 should explicitly reference the paper from which they are
taken (as we do with Fig 14).


**** TAPIO ****


o Thanks Tapio Helin in the introduction.


o p10 YES

o p12 define weak convergence of probability measures notation in Notation
section of introduction.

o p18 YES

o p41 YES

o p47 yes mathbbm{1}

o p57 yes

o p58 yes. both.

o p59 expand to say:

"Since we assumed that $\rho_0'=\rho$, with $\rho$ the invariant meausure,
it follows that $\rho_k'=\rho$ for all $k$..."

o p59 others all minor typos: yes

o p62 State that as a consequence what Ta[io writes follows.

o p64 yes

o p65 yes

o p67 i think i'd already expanded on this.

o p69 yes and the rank condition is used in proof of C9.5 only (please state)

o p71 yes

o p72 yes

o p73 i think i caucht this; pls check

o p75 yes

o p76 explain that e_0 is the initial error but that its value is irrelevant
when taking j --> infty

o p79 yes first comment, the second i'd caught and rewritten, the thrid yes.

o p80 yes

o p81 yes







